Incorporating Connectivity among Internet Search Data for Enhanced Influenza-like Illness Tracking

Big data collected from the Internet possess great potential to reveal the ever-changing trends in society. In particular, accurate infectious disease tracking with Internet data has grown in popularity, providing invaluable information for public health decision makers and the general public. However, much of the complex connectivity among the Internet search data is not effectively addressed among existing disease tracking frameworks. To this end, we propose ARGO-C (Augmented Regression with Clustered GOogle data), an integrative, statistically principled approach that incorporates the clustering structure of Internet search data to enhance the accuracy and interpretability of disease tracking. Focusing on multi-resolution %ILI (influenza-like illness) tracking, we demonstrate the improved performance and robustness of ARGO-C over benchmark methods at various geographical resolutions. We also highlight the adaptability of ARGO-C to track various diseases in addition to influenza, and to track other social or economic trends.

==> figs/tables_state_error.tex <==
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & \textbf{0.831} & \textbf{0.752} & \textbf{0.577} & \textbf{1.756} & \textbf{1.922} & 0.625 & \textbf{0.544} & \textbf{0.846} & \textbf{0.504} & \textbf{0.698} & 0.198 & \textbf{0.274} & \textbf{1.507} \\ 
  ARGOX & 0.873 & 0.797 & 0.632 & 1.865 & 2.045 & 0.607 & 0.596 & 0.864 & 0.530 & 0.779 & 0.192 & 0.289 & 1.653 \\ 
  VAR1 & 2.407 & 2.383 & 2.336 & 4.624 & 5.083 & 1.324 & 2.231 & 3.394 & 1.693 & 3.559 & 0.351 & 0.687 & 5.138 \\ 
  GFT & -- & -- & -- & 2.891 & 3.183 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 1.115 & 0.977 & 0.646 & 2.271 & 2.495 & \textbf{0.591} & 0.831 & 1.315 & 0.785 & 1.043 & \textbf{0.142} & 0.453 & 1.645 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & \textbf{0.462} & \textbf{0.400} & \textbf{0.284} & \textbf{1.107} & \textbf{1.262} & 0.480 & \textbf{0.407} & \textbf{0.459} & \textbf{0.342} & \textbf{0.492} & 0.155 & 0.213 & \textbf{1.067} \\ 
  ARGOX & 0.477 & 0.413 & 0.294 & 1.119 & 1.292 & 0.463 & 0.467 & 0.482 & 0.369 & 0.530 & 0.154 & \textbf{0.196} & 1.210 \\ 
  VAR1 & 1.349 & 1.271 & 1.125 & 2.847 & 3.324 & 1.156 & 1.665 & 2.169 & 1.072 & 2.374 & 0.293 & 0.599 & 4.203 \\ 
  GFT & -- & -- & -- & 1.934 & 2.321 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.595 & 0.501 & 0.325 & 1.316 & 1.552 & \textbf{0.444} & 0.639 & 0.757 & 0.573 & 0.782 & \textbf{0.121} & 0.307 & 1.189 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & \textbf{ 0.956} & \textbf{ 0.956} & \textbf{ 0.945} &  0.911 &  0.894 &  0.815 & \textbf{ 0.958} & \textbf{ 0.976} & \textbf{ 0.970} & \textbf{ 0.962} &  0.709 & \textbf{ 0.980} & \textbf{ 0.832} \\ 
  ARGOX &  0.952 &  0.951 &  0.936 &  0.898 &  0.878 &  0.831 &  0.950 &  0.976 &  0.966 &  0.951 &  0.721 &  0.970 &  0.799 \\ 
  VAR1 &  0.675 &  0.517 &  0.632 &  0.715 &  0.655 &  0.820 &  0.639 &  0.615 &  0.859 &  0.278 & -0.105 &  0.777 & -0.040 \\ 
  GFT & -- & -- & -- & \textbf{ 0.960} & \textbf{ 0.952} & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive &  0.923 &  0.928 &  0.933 &  0.855 &  0.826 & \textbf{ 0.851} &  0.906 &  0.941 &  0.925 &  0.908 & \textbf{ 0.795} &  0.906 &  0.808 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in Alabama.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.AL}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & \textbf{0.961} & \textbf{0.849} & \textbf{0.586} & 0.663 & 0.630 & \textbf{0.828} & \textbf{0.705} & \textbf{0.634} & \textbf{1.097} & 1.962 & 0.301 & \textbf{0.631} & \textbf{0.625} \\ 
  ARGOX & 0.966 & 0.855 & 0.596 & 0.654 & 0.622 & 0.832 & 0.707 & 0.635 & 1.108 & 1.979 & 0.298 & 0.655 & 0.630 \\ 
  VAR1 & 1.058 & 0.945 & 0.690 & 0.689 & 0.656 & 1.159 & 0.929 & 1.095 & 1.215 & \textbf{1.847} & 0.305 & 0.789 & 1.071 \\ 
  GFT & -- & -- & -- & 1.015 & 1.042 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 1.002 & 0.896 & 0.654 & \textbf{0.646} & \textbf{0.605} & 0.843 & 0.783 & 0.645 & 1.126 & 2.047 & \textbf{0.287} & 0.788 & 0.660 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & \textbf{0.594} & \textbf{0.519} & \textbf{0.381} & 0.493 & 0.460 & \textbf{0.565} & \textbf{0.519} & \textbf{0.508} & \textbf{0.765} & 1.267 & 0.208 & 0.363 & 0.437 \\ 
  ARGOX & 0.595 & 0.521 & 0.382 & 0.488 & 0.454 & 0.569 & 0.524 & 0.515 & 0.774 & 1.265 & \textbf{0.200} & \textbf{0.361} & \textbf{0.436} \\ 
  VAR1 & 0.684 & 0.601 & 0.449 & 0.538 & 0.502 & 0.749 & 0.686 & 0.938 & 0.836 & \textbf{1.148} & 0.214 & 0.447 & 0.860 \\ 
  GFT & -- & -- & -- & 0.867 & 0.877 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.619 & 0.552 & 0.429 & \textbf{0.479} & \textbf{0.438} & 0.596 & 0.604 & 0.519 & 0.821 & 1.259 & 0.210 & 0.479 & 0.485 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & \textbf{0.871} & \textbf{0.873} & \textbf{0.821} & 0.731 & 0.777 & 0.818 & \textbf{0.796} & \textbf{0.915} & \textbf{0.881} & \textbf{0.629} & 0.604 & \textbf{0.795} & \textbf{0.838} \\ 
  ARGOX & 0.870 & 0.871 & 0.808 & 0.737 & 0.782 & 0.816 & 0.796 & 0.914 & 0.879 & 0.620 & \textbf{0.605} & 0.782 & 0.828 \\ 
  VAR1 & 0.856 & 0.851 & 0.701 & 0.756 & 0.807 & 0.802 & 0.743 & 0.893 & 0.870 & 0.614 & 0.552 & 0.741 & 0.678 \\ 
  GFT & -- & -- & -- & 0.623 & 0.776 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.864 & 0.864 & 0.774 & \textbf{0.768} & \textbf{0.812} & \textbf{0.820} & 0.769 & 0.907 & 0.880 & 0.603 & 0.533 & 0.712 & 0.759 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in Alaska.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.AK}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & \textbf{0.396} & \textbf{0.378} & 0.342 & \textbf{0.246} & \textbf{0.256} & \textbf{0.391} & 0.319 & \textbf{0.587} & 0.315 & 0.662 & 0.272 & 0.336 & \textbf{0.483} \\ 
  ARGOX & 0.404 & 0.382 & \textbf{0.338} & 0.253 & 0.266 & 0.413 & 0.311 & 0.645 & \textbf{0.309} & \textbf{0.629} & \textbf{0.259} & \textbf{0.335} & 0.513 \\ 
  VAR1 & 2.372 & 2.080 & 1.384 & 4.487 & 4.938 & 1.218 & 2.423 & 2.891 & 1.615 & 2.398 & 0.365 & 0.539 & 3.543 \\ 
  GFT & -- & -- & -- & 1.160 & 1.253 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.454 & 0.432 & 0.387 & 0.280 & 0.298 & 0.401 & \textbf{0.304} & 0.787 & 0.363 & 0.707 & 0.279 & 0.424 & 0.679 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & \textbf{0.290} & \textbf{0.277} & 0.254 & 0.187 & 0.193 & \textbf{0.286} & 0.267 & \textbf{0.448} & 0.267 & 0.533 & 0.227 & \textbf{0.243} & \textbf{0.370} \\ 
  ARGOX & 0.292 & 0.278 & \textbf{0.251} & \textbf{0.182} & \textbf{0.192} & 0.304 & 0.259 & 0.484 & \textbf{0.266} & \textbf{0.505} & \textbf{0.212} & 0.246 & 0.401 \\ 
  VAR1 & 1.409 & 1.164 & 0.708 & 2.910 & 3.479 & 0.976 & 1.960 & 1.892 & 0.976 & 1.839 & 0.316 & 0.343 & 2.430 \\ 
  GFT & -- & -- & -- & 1.010 & 1.131 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.309 & 0.294 & 0.266 & 0.216 & 0.233 & 0.293 & \textbf{0.254} & 0.539 & 0.269 & 0.542 & 0.217 & 0.292 & 0.525 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & \textbf{0.953} & \textbf{0.952} & 0.938 & \textbf{0.959} & \textbf{0.955} & \textbf{0.945} & 0.862 & \textbf{0.942} & 0.921 & 0.846 & 0.770 & \textbf{0.888} & \textbf{0.954} \\ 
  ARGOX & 0.951 & 0.951 & \textbf{0.940} & 0.958 & 0.953 & 0.938 & 0.864 & 0.928 & \textbf{0.925} & \textbf{0.855} & \textbf{0.780} & 0.882 & 0.945 \\ 
  VAR1 & 0.613 & 0.660 & 0.754 & 0.725 & 0.666 & 0.468 & 0.680 & 0.719 & 0.707 & 0.799 & 0.516 & 0.861 & 0.484 \\ 
  GFT & -- & -- & -- & 0.923 & 0.912 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.939 & 0.939 & 0.924 & 0.941 & 0.932 & 0.939 & \textbf{0.865} & 0.884 & 0.901 & 0.816 & 0.749 & 0.816 & 0.904 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in Arizona.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.AZ}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & \textbf{0.821} & \textbf{0.741} & \textbf{0.564} & \textbf{1.050} & \textbf{1.144} & 0.622 & \textbf{0.842} & \textbf{0.905} & 0.830 & \textbf{1.576} & 0.195 & 0.405 & \textbf{0.718} \\ 
  ARGOX & 0.853 & 0.780 & 0.622 & 1.102 & 1.201 & \textbf{0.612} & 0.897 & 0.973 & \textbf{0.805} & 1.716 & 0.199 & \textbf{0.382} & 0.798 \\ 
  VAR1 & 1.103 & 0.950 & 0.565 & 1.382 & 1.514 & 0.656 & 1.154 & 1.597 & 1.041 & 1.812 & \textbf{0.167} & 0.417 & 0.885 \\ 
  GFT & -- & -- & -- & 1.391 & 1.466 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 1.049 & 0.919 & 0.609 & 1.328 & 1.453 & 0.647 & 1.080 & 1.444 & 0.987 & 1.871 & 0.168 & 0.421 & 0.846 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & \textbf{0.518} & \textbf{0.450} & 0.324 & \textbf{0.601} & \textbf{0.657} & 0.456 & \textbf{0.596} & \textbf{0.698} & \textbf{0.569} & \textbf{1.159} & 0.155 & 0.292 & \textbf{0.579} \\ 
  ARGOX & 0.530 & 0.463 & 0.339 & 0.649 & 0.716 & \textbf{0.446} & 0.605 & 0.732 & 0.584 & 1.228 & 0.159 & \textbf{0.274} & 0.672 \\ 
  VAR1 & 0.636 & 0.521 & \textbf{0.306} & 0.809 & 0.923 & 0.464 & 0.713 & 1.012 & 0.771 & 1.202 & 0.142 & 0.309 & 0.729 \\ 
  GFT & -- & -- & -- & 1.179 & 1.237 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.627 & 0.518 & 0.316 & 0.747 & 0.847 & 0.472 & 0.708 & 1.042 & 0.729 & 1.253 & \textbf{0.136} & 0.326 & 0.704 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & \textbf{0.946} & \textbf{0.943} & \textbf{0.923} & 0.922 & 0.907 & 0.865 & \textbf{0.937} & \textbf{0.975} & 0.938 & \textbf{0.826} & 0.722 & \textbf{0.859} & \textbf{0.927} \\ 
  ARGOX & 0.942 & 0.937 & 0.910 & 0.913 & 0.896 & \textbf{0.872} & 0.928 & 0.969 & \textbf{0.940} & 0.795 & \textbf{0.723} & 0.856 & 0.910 \\ 
  VAR1 & 0.911 & 0.908 & 0.914 & 0.877 & 0.853 & 0.860 & 0.885 & 0.914 & 0.899 & 0.753 & 0.712 & 0.814 & 0.892 \\ 
  GFT & -- & -- & -- & \textbf{0.971} & \textbf{0.967} & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.913 & 0.914 & 0.911 & 0.878 & 0.854 & 0.866 & 0.893 & 0.918 & 0.903 & 0.755 & 0.711 & 0.812 & 0.900 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in Arkansas.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.AR}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & \textbf{0.252} & \textbf{0.267} & \textbf{0.292} & \textbf{0.255} & \textbf{0.275} & \textbf{0.278} & 0.247 & \textbf{0.389} & 0.235 & 0.342 & 0.142 & \textbf{0.248} & \textbf{0.649} \\ 
  ARGOX & 0.260 & 0.279 & 0.312 & 0.276 & 0.298 & 0.303 & \textbf{0.243} & 0.416 & \textbf{0.217} & \textbf{0.326} & \textbf{0.133} & 0.261 & 0.738 \\ 
  VAR1 & 0.793 & 0.872 & 1.003 & 1.287 & 1.347 & 0.648 & 0.640 & 0.987 & 0.595 & 0.810 & 0.264 & 0.671 & 2.477 \\ 
  GFT & -- & -- & -- & 0.535 & 0.555 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.344 & 0.372 & 0.419 & 0.370 & 0.402 & 0.354 & 0.252 & 0.640 & 0.262 & 0.492 & 0.150 & 0.410 & 0.937 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & 0.182 & \textbf{0.185} & \textbf{0.192} & \textbf{0.197} & \textbf{0.216} & \textbf{0.219} & \textbf{0.179} & \textbf{0.263} & 0.188 & 0.251 & 0.115 & \textbf{0.206} & \textbf{0.513} \\ 
  ARGOX & \textbf{0.181} & 0.186 & 0.194 & 0.205 & 0.225 & 0.241 & 0.183 & 0.274 & \textbf{0.165} & \textbf{0.239} & \textbf{0.109} & 0.208 & 0.559 \\ 
  VAR1 & 0.636 & 0.646 & 0.665 & 1.206 & 1.264 & 0.472 & 0.570 & 0.836 & 0.475 & 0.620 & 0.206 & 0.513 & 2.311 \\ 
  GFT & -- & -- & -- & 0.398 & 0.400 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.220 & 0.228 & 0.244 & 0.247 & 0.275 & 0.277 & 0.194 & 0.390 & 0.220 & 0.347 & 0.119 & 0.243 & 0.739 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & \textbf{0.974} & \textbf{0.977} & \textbf{0.981} & \textbf{0.967} & \textbf{0.961} & \textbf{0.942} & \textbf{0.934} & \textbf{0.959} & 0.950 & 0.970 & 0.947 & \textbf{0.955} & \textbf{0.953} \\ 
  ARGOX & 0.972 & 0.975 & 0.978 & 0.963 & 0.956 & 0.930 & 0.930 & 0.953 & \textbf{0.959} & \textbf{0.973} & \textbf{0.952} & 0.948 & 0.933 \\ 
  VAR1 & 0.774 & 0.750 & 0.812 & 0.902 & 0.883 & 0.879 & 0.482 & 0.902 & 0.853 & 0.836 & 0.807 & 0.597 & 0.900 \\ 
  GFT & -- & -- & -- & 0.941 & 0.936 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.952 & 0.956 & 0.960 & 0.928 & 0.914 & 0.907 & 0.917 & 0.889 & 0.940 & 0.934 & 0.940 & 0.873 & 0.890 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in California.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.CA}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & 0.422 & \textbf{0.410} & \textbf{0.386} & 0.410 & 0.450 & \textbf{0.151} & 0.608 & 0.225 & 0.790 & \textbf{0.422} & 0.150 & \textbf{0.370} & \textbf{0.862} \\ 
  ARGOX & \textbf{0.417} & 0.411 & 0.401 & \textbf{0.402} & \textbf{0.441} & 0.155 & \textbf{0.589} & \textbf{0.207} & 0.783 & 0.443 & 0.146 & 0.384 & 0.906 \\ 
  VAR1 & 1.414 & 1.289 & 1.019 & 1.671 & 1.669 & 1.512 & 0.880 & 1.602 & 1.921 & 1.829 & 0.621 & 1.340 & 1.582 \\ 
  GFT & -- & -- & -- & 0.809 & 0.886 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.461 & 0.489 & 0.536 & 0.478 & 0.525 & 0.208 & 0.685 & 0.270 & \textbf{0.725} & 0.829 & \textbf{0.130} & 0.376 & 1.143 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & 0.272 & 0.262 & \textbf{0.244} & \textbf{0.242} & \textbf{0.279} & 0.117 & 0.445 & 0.180 & 0.629 & \textbf{0.305} & 0.117 & 0.281 & \textbf{0.673} \\ 
  ARGOX & \textbf{0.270} & \textbf{0.262} & 0.248 & 0.245 & 0.282 & \textbf{0.113} & \textbf{0.436} & \textbf{0.156} & 0.621 & 0.332 & 0.114 & \textbf{0.276} & 0.706 \\ 
  VAR1 & 1.202 & 1.039 & 0.735 & 1.611 & 1.599 & 1.438 & 0.771 & 1.368 & 1.624 & 1.488 & 0.429 & 1.162 & 1.242 \\ 
  GFT & -- & -- & -- & 0.458 & 0.514 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.303 & 0.305 & 0.309 & 0.304 & 0.352 & 0.166 & 0.506 & 0.216 & \textbf{0.562} & 0.596 & \textbf{0.100} & 0.303 & 0.915 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C &  0.970 & \textbf{ 0.975} & \textbf{ 0.981} &  0.930 &  0.921 & \textbf{ 0.939} &  0.450 &  0.977 & \textbf{ 0.913} & \textbf{ 0.983} &  0.866 & \textbf{ 0.918} & \textbf{ 0.955} \\ 
  ARGOX & \textbf{ 0.971} &  0.974 &  0.979 & \textbf{ 0.933} & \textbf{ 0.924} &  0.935 &  0.481 & \textbf{ 0.980} &  0.913 &  0.982 & \textbf{ 0.875} &  0.913 &  0.949 \\ 
  VAR1 &  0.630 &  0.725 &  0.864 &  0.854 &  0.832 &  0.865 & \textbf{ 0.626} &  0.790 &  0.846 &  0.872 & -0.210 &  0.189 &  0.849 \\ 
  GFT & -- & -- & -- &  0.841 &  0.816 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive &  0.964 &  0.964 &  0.964 &  0.902 &  0.886 &  0.885 &  0.374 &  0.959 &  0.904 &  0.930 &  0.854 &  0.903 &  0.917 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in Colorado.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.CO}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & \textbf{0.534} & \textbf{0.489} & \textbf{0.393} & 0.677 & 0.743 & 0.471 & 0.409 & 0.462 & 0.445 & \textbf{0.724} & 0.162 & \textbf{0.337} & \textbf{0.734} \\ 
  ARGOX & 0.536 & 0.493 & 0.400 & 0.680 & 0.746 & 0.471 & \textbf{0.395} & \textbf{0.447} & \textbf{0.412} & 0.769 & 0.158 & 0.371 & 0.762 \\ 
  VAR1 & 1.425 & 1.274 & 0.933 & 1.684 & 1.840 & 1.548 & 1.589 & 2.358 & 0.828 & 1.163 & 0.267 & 1.012 & 2.018 \\ 
  GFT & -- & -- & -- & 1.475 & 1.614 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.576 & 0.537 & 0.456 & \textbf{0.625} & \textbf{0.683} & \textbf{0.462} & 0.492 & 0.575 & 0.493 & 0.865 & \textbf{0.149} & 0.414 & 0.935 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & 0.365 & 0.316 & \textbf{0.226} & 0.440 & 0.514 & 0.376 & 0.314 & 0.351 & 0.352 & 0.543 & 0.127 & \textbf{0.211} & \textbf{0.520} \\ 
  ARGOX & \textbf{0.358} & \textbf{0.313} & 0.231 & 0.433 & 0.504 & 0.382 & \textbf{0.300} & \textbf{0.336} & \textbf{0.311} & \textbf{0.540} & 0.120 & 0.221 & 0.575 \\ 
  VAR1 & 1.078 & 0.907 & 0.589 & 1.311 & 1.496 & 1.363 & 1.253 & 2.055 & 0.614 & 1.020 & 0.220 & 0.865 & 1.595 \\ 
  GFT & -- & -- & -- & 1.092 & 1.254 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.376 & 0.336 & 0.261 & \textbf{0.348} & \textbf{0.388} & \textbf{0.360} & 0.379 & 0.423 & 0.367 & 0.640 & \textbf{0.110} & 0.281 & 0.741 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & 0.959 & \textbf{0.963} & \textbf{0.972} & 0.901 & 0.874 & 0.884 & 0.948 & 0.966 & 0.946 & \textbf{0.967} & \textbf{0.904} & \textbf{0.937} & \textbf{0.935} \\ 
  ARGOX & \textbf{0.959} & 0.963 & 0.970 & 0.901 & 0.875 & 0.881 & \textbf{0.952} & \textbf{0.968} & \textbf{0.954} & 0.965 & 0.903 & 0.913 & 0.928 \\ 
  VAR1 & 0.729 & 0.755 & 0.907 & 0.642 & 0.564 & 0.697 & 0.679 & 0.950 & 0.840 & 0.902 & 0.598 & 0.697 & 0.904 \\ 
  GFT & -- & -- & -- & 0.748 & 0.686 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.952 & 0.956 & 0.963 & \textbf{0.914} & \textbf{0.894} & \textbf{0.887} & 0.925 & 0.948 & 0.934 & 0.945 & 0.898 & 0.850 & 0.889 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in Connecticut.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.CT}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & \textbf{0.421} & \textbf{0.404} & \textbf{0.370} & 0.549 & 0.604 & 0.252 & 0.203 & 0.689 & 0.256 & \textbf{0.808} & 0.190 & \textbf{0.293} & \textbf{0.315} \\ 
  ARGOX & 0.421 & 0.405 & 0.373 & 0.553 & 0.608 & \textbf{0.243} & \textbf{0.186} & \textbf{0.684} & \textbf{0.254} & 0.836 & \textbf{0.186} & 0.295 & 0.324 \\ 
  VAR1 & 1.898 & 1.755 & 1.453 & 1.747 & 1.882 & 1.808 & 2.227 & 2.454 & 2.420 & 3.279 & 0.426 & 0.696 & 2.519 \\ 
  GFT & -- & -- & -- & 2.085 & 2.232 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.453 & 0.453 & 0.452 & \textbf{0.509} & \textbf{0.560} & 0.256 & 0.230 & 0.785 & 0.293 & 0.954 & 0.202 & 0.376 & 0.502 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & 0.217 & \textbf{0.218} & \textbf{0.221} & 0.272 & 0.320 & 0.189 & 0.159 & 0.372 & \textbf{0.196} & \textbf{0.547} & 0.153 & \textbf{0.229} & 0.254 \\ 
  ARGOX & \textbf{0.217} & 0.218 & 0.222 & 0.280 & 0.330 & 0.184 & \textbf{0.147} & \textbf{0.354} & 0.201 & 0.561 & \textbf{0.151} & 0.235 & \textbf{0.254} \\ 
  VAR1 & 1.529 & 1.302 & 0.880 & 1.504 & 1.644 & 1.659 & 2.022 & 2.240 & 2.300 & 2.877 & 0.374 & 0.586 & 2.096 \\ 
  GFT & -- & -- & -- & 1.880 & 2.032 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.226 & 0.233 & 0.247 & \textbf{0.245} & \textbf{0.288} & \textbf{0.173} & 0.173 & 0.468 & 0.208 & 0.618 & 0.163 & 0.277 & 0.396 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & \textbf{0.873} & \textbf{0.887} & \textbf{0.896} & 0.825 & 0.811 & 0.829 & 0.767 & 0.883 & 0.907 & \textbf{0.809} & 0.661 & \textbf{0.897} & \textbf{0.935} \\ 
  ARGOX & 0.873 & 0.886 & 0.894 & 0.823 & 0.809 & \textbf{0.840} & 0.810 & \textbf{0.885} & \textbf{0.912} & 0.800 & 0.671 & 0.883 & 0.932 \\ 
  VAR1 & 0.708 & 0.671 & 0.709 & 0.449 & 0.380 & 0.494 & \textbf{0.835} & 0.781 & 0.775 & 0.609 & \textbf{0.735} & 0.845 & 0.875 \\ 
  GFT & -- & -- & -- & 0.737 & 0.714 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.859 & 0.864 & 0.846 & \textbf{0.859} & \textbf{0.847} & 0.832 & 0.739 & 0.848 & 0.882 & 0.735 & 0.638 & 0.809 & 0.844 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in Delaware.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.DE}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & 1.421 & 1.264 & 0.904 & 1.515 & 1.596 & \textbf{1.595} & \textbf{2.054} & 1.190 & 0.494 & 0.802 & 0.508 & 0.728 & 1.660 \\ 
  ARGOX & \textbf{1.418} & \textbf{1.262} & 0.902 & \textbf{1.509} & \textbf{1.587} & 1.615 & 2.062 & 1.226 & \textbf{0.459} & 0.798 & 0.512 & \textbf{0.714} & 1.673 \\ 
  VAR1 & 1.523 & 1.346 & 0.934 & 1.560 & 1.651 & 1.632 & 2.157 & 1.604 & 0.542 & 0.861 & \textbf{0.459} & 0.777 & 1.601 \\ 
  GFT & -- & -- & -- & 5.236 & 5.015 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 1.447 & 1.276 & \textbf{0.872} & 1.588 & 1.676 & 1.669 & 2.193 & \textbf{0.846} & 0.529 & \textbf{0.770} & 0.496 & 0.796 & \textbf{1.465} \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & 0.977 & 0.860 & 0.645 & 1.153 & 1.200 & 1.329 & \textbf{1.422} & 0.956 & 0.348 & 0.647 & 0.352 & 0.561 & 1.409 \\ 
  ARGOX & 0.978 & 0.863 & 0.648 & \textbf{1.148} & \textbf{1.198} & 1.295 & 1.447 & 1.018 & \textbf{0.315} & 0.642 & 0.380 & \textbf{0.546} & 1.432 \\ 
  VAR1 & 1.069 & 0.925 & 0.657 & 1.220 & 1.289 & \textbf{1.265} & 1.505 & 1.483 & 0.438 & 0.638 & 0.338 & 0.588 & 1.313 \\ 
  GFT & -- & -- & -- & 4.935 & 4.686 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & \textbf{0.890} & \textbf{0.788} & \textbf{0.601} & 1.274 & 1.342 & 1.277 & 1.509 & \textbf{0.453} & 0.342 & \textbf{0.607} & \textbf{0.335} & 0.606 & \textbf{1.224} \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & \textbf{0.874} & 0.886 & 0.923 & 0.831 & 0.848 & 0.797 & \textbf{0.601} & 0.649 & 0.642 & 0.731 & \textbf{0.432} & \textbf{0.745} & 0.847 \\ 
  ARGOX & 0.874 & 0.886 & 0.924 & \textbf{0.832} & \textbf{0.851} & 0.791 & 0.592 & 0.664 & \textbf{0.688} & 0.738 & 0.403 & 0.742 & 0.846 \\ 
  VAR1 & 0.850 & 0.867 & 0.924 & 0.807 & 0.819 & \textbf{0.816} & 0.552 & 0.557 & 0.486 & 0.774 & 0.398 & 0.700 & 0.864 \\ 
  GFT & -- & -- & -- & 0.766 & 0.833 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.873 & \textbf{0.888} & \textbf{0.928} & 0.816 & 0.828 & 0.810 & 0.562 & \textbf{0.721} & 0.605 & \textbf{0.787} & 0.390 & 0.700 & \textbf{0.884} \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in District of Columbia.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.DC}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & \textbf{0.577} & \textbf{0.543} & \textbf{0.473} & 0.860 & 0.945 & \textbf{0.318} & \textbf{0.421} & 1.031 & \textbf{0.401} & \textbf{0.700} & 0.247 & \textbf{0.446} & \textbf{0.856} \\ 
  ARGOX & 0.593 & 0.560 & 0.492 & 0.871 & 0.957 & 0.330 & 0.437 & \textbf{1.017} & 0.459 & 0.753 & 0.249 & 0.482 & 0.951 \\ 
  VAR1 & 3.205 & 2.992 & 2.550 & 2.220 & 2.421 & 1.629 & 3.280 & 5.718 & 3.521 & 4.928 & 1.583 & 2.289 & 4.099 \\ 
  GFT & -- & -- & -- & \textbf{0.819} & \textbf{0.896} & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.816 & 0.758 & 0.638 & 0.999 & 1.098 & 0.358 & 0.564 & 1.501 & 0.672 & 1.360 & \textbf{0.206} & 0.740 & 0.935 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & \textbf{0.330} & \textbf{0.326} & \textbf{0.318} & \textbf{0.418} & \textbf{0.480} & \textbf{0.239} & \textbf{0.343} & 0.622 & \textbf{0.300} & \textbf{0.544} & 0.204 & 0.313 & \textbf{0.655} \\ 
  ARGOX & 0.339 & 0.332 & 0.319 & 0.430 & 0.497 & 0.243 & 0.368 & \textbf{0.600} & 0.314 & 0.574 & 0.201 & \textbf{0.292} & 0.739 \\ 
  VAR1 & 2.431 & 2.339 & 2.170 & 1.560 & 1.741 & 1.554 & 3.056 & 4.344 & 3.335 & 4.445 & 1.539 & 1.950 & 3.503 \\ 
  GFT & -- & -- & -- & 0.505 & 0.574 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.430 & 0.419 & 0.397 & 0.486 & 0.564 & 0.275 & 0.418 & 0.856 & 0.488 & 1.041 & \textbf{0.164} & 0.461 & 0.700 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & \textbf{ 0.970} & \textbf{ 0.968} & \textbf{ 0.961} &  0.864 &  0.845 & \textbf{ 0.870} & \textbf{ 0.950} &  0.969 & \textbf{ 0.961} & \textbf{ 0.965} &  0.841 & \textbf{ 0.971} & \textbf{ 0.897} \\ 
  ARGOX &  0.969 &  0.966 &  0.958 &  0.854 &  0.833 &  0.866 &  0.947 & \textbf{ 0.970} &  0.950 &  0.960 &  0.828 &  0.960 &  0.874 \\ 
  VAR1 &  0.543 &  0.551 &  0.662 &  0.185 &  0.093 &  0.622 &  0.665 &  0.526 &  0.647 &  0.587 &  0.423 &  0.770 & -0.188 \\ 
  GFT & -- & -- & -- & \textbf{ 0.892} & \textbf{ 0.877} & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive &  0.941 &  0.939 &  0.929 &  0.812 &  0.787 &  0.837 &  0.909 &  0.933 &  0.878 &  0.858 & \textbf{ 0.872} &  0.885 &  0.869 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in Georgia.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.GA}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & \textbf{0.903} & \textbf{0.775} & 0.450 & 1.659 & 1.702 & \textbf{0.769} & 0.688 & \textbf{1.155} & \textbf{0.611} & 0.648 & 0.354 & 0.349 & \textbf{0.471} \\ 
  ARGOX & 0.906 & 0.778 & 0.453 & 1.660 & 1.704 & 0.773 & \textbf{0.684} & 1.164 & 0.625 & 0.643 & \textbf{0.350} & 0.356 & 0.485 \\ 
  VAR1 & 2.945 & 2.647 & 1.978 & 5.999 & 6.525 & 1.870 & 0.973 & 3.918 & 1.713 & 3.541 & 1.481 & 1.985 & 2.306 \\ 
  GFT & -- & -- & -- & 4.131 & 4.457 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.930 & 0.796 & \textbf{0.449} & \textbf{1.597} & \textbf{1.627} & 0.787 & 0.740 & 1.269 & 0.707 & \textbf{0.618} & 0.374 & \textbf{0.347} & 0.504 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & \textbf{0.618} & \textbf{0.517} & 0.330 & 1.132 & 1.185 & \textbf{0.611} & 0.568 & 0.865 & \textbf{0.468} & 0.487 & 0.297 & 0.241 & \textbf{0.369} \\ 
  ARGOX & 0.620 & 0.519 & 0.332 & 1.137 & 1.192 & 0.621 & \textbf{0.564} & \textbf{0.861} & 0.474 & 0.492 & \textbf{0.295} & 0.246 & 0.379 \\ 
  VAR1 & 1.636 & 1.632 & 1.623 & 4.806 & 5.521 & 1.371 & 0.747 & 2.152 & 1.262 & 2.811 & 1.397 & 1.668 & 1.804 \\ 
  GFT & -- & -- & -- & 3.590 & 3.997 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.654 & 0.540 & \textbf{0.328} & \textbf{1.100} & \textbf{1.153} & 0.642 & 0.609 & 0.977 & 0.510 & \textbf{0.475} & 0.311 & \textbf{0.236} & 0.398 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & \textbf{ 0.935} & \textbf{ 0.942} &  0.925 &  0.915 &  0.900 & \textbf{ 0.907} & \textbf{ 0.745} & \textbf{ 0.770} & \textbf{ 0.870} & \textbf{ 0.905} &  0.108 &  0.862 & \textbf{ 0.558} \\ 
  ARGOX &  0.934 &  0.942 &  0.924 &  0.915 &  0.901 &  0.905 &  0.743 &  0.762 &  0.864 &  0.901 &  0.111 &  0.860 &  0.532 \\ 
  VAR1 &  0.299 &  0.310 &  0.700 &  0.490 &  0.399 &  0.796 &  0.708 &  0.528 &  0.457 &  0.491 & -0.050 &  0.614 &  0.445 \\ 
  GFT & -- & -- & -- &  0.906 & \textbf{ 0.942} & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive &  0.932 &  0.940 & \textbf{ 0.927} & \textbf{ 0.923} &  0.908 &  0.905 &  0.716 &  0.721 &  0.833 &  0.890 & \textbf{ 0.113} & \textbf{ 0.865} &  0.470 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in Hawaii.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.HI}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & 0.508 & \textbf{0.622} & \textbf{0.791} & 0.651 & 0.670 & 0.530 & \textbf{0.411} & 0.568 & \textbf{0.730} & 0.906 & 0.233 & 0.578 & \textbf{1.475} \\ 
  ARGOX & \textbf{0.495} & 0.623 & 0.809 & \textbf{0.632} & \textbf{0.651} & 0.499 & 0.420 & \textbf{0.519} & 0.739 & 0.938 & \textbf{0.231} & \textbf{0.569} & 1.515 \\ 
  VAR1 & 2.281 & 2.027 & 1.443 & 4.065 & 4.298 & 2.339 & 1.798 & 2.449 & 1.559 & 1.851 & 0.500 & 1.146 & 3.160 \\ 
  GFT & -- & -- & -- & 1.243 & 1.355 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.566 & 0.669 & 0.826 & 0.827 & 0.850 & \textbf{0.470} & 0.478 & 0.639 & 0.820 & \textbf{0.808} & 0.234 & 0.595 & 1.672 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & 0.361 & 0.394 & 0.456 & 0.475 & 0.477 & 0.435 & 0.330 & 0.429 & \textbf{0.522} & 0.622 & 0.153 & 0.405 & \textbf{0.976} \\ 
  ARGOX & \textbf{0.347} & \textbf{0.389} & 0.465 & \textbf{0.451} & \textbf{0.452} & 0.401 & \textbf{0.329} & \textbf{0.388} & 0.527 & 0.643 & \textbf{0.146} & 0.398 & 1.018 \\ 
  VAR1 & 1.860 & 1.545 & 0.962 & 3.381 & 3.654 & 1.923 & 1.676 & 2.294 & 1.379 & 1.624 & 0.403 & 0.938 & 2.588 \\ 
  GFT & -- & -- & -- & 1.035 & 1.168 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.380 & 0.402 & \textbf{0.442} & 0.623 & 0.632 & \textbf{0.375} & 0.362 & 0.474 & 0.583 & \textbf{0.528} & 0.162 & \textbf{0.376} & 1.128 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C &  0.916 & \textbf{ 0.900} & \textbf{ 0.871} &  0.939 &  0.931 &  0.563 & \textbf{ 0.801} &  0.846 & \textbf{ 0.786} &  0.685 &  0.808 &  0.645 & \textbf{ 0.902} \\ 
  ARGOX & \textbf{ 0.920} &  0.899 &  0.864 &  0.941 &  0.933 &  0.611 &  0.786 & \textbf{ 0.870} &  0.778 &  0.669 &  0.814 &  0.653 &  0.891 \\ 
  VAR1 &  0.794 &  0.508 &  0.528 &  0.719 &  0.652 &  0.587 &  0.637 &  0.791 &  0.679 & -0.270 &  0.428 &  0.283 &  0.430 \\ 
  GFT & -- & -- & -- & \textbf{ 0.953} & \textbf{ 0.955} & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive &  0.899 &  0.890 &  0.868 &  0.901 &  0.888 & \textbf{ 0.692} &  0.750 &  0.814 &  0.754 & \textbf{ 0.781} & \textbf{ 0.822} & \textbf{ 0.674} &  0.867 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in Idaho.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.ID}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & \textbf{0.284} & \textbf{0.284} & \textbf{0.284} & 0.460 & 0.503 & 0.233 & \textbf{0.230} & \textbf{0.328} & \textbf{0.269} & \textbf{0.430} & 0.156 & 0.293 & \textbf{0.555} \\ 
  ARGOX & 0.291 & 0.292 & 0.292 & \textbf{0.443} & \textbf{0.485} & \textbf{0.233} & 0.241 & 0.354 & 0.272 & 0.471 & 0.146 & \textbf{0.273} & 0.615 \\ 
  VAR1 & 1.628 & 1.552 & 1.399 & 2.173 & 2.332 & 1.926 & 1.832 & 1.962 & 0.955 & 2.258 & 0.715 & 0.730 & 2.283 \\ 
  GFT & -- & -- & -- & 0.672 & 0.704 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.401 & 0.396 & 0.387 & 0.459 & 0.501 & 0.271 & 0.360 & 0.626 & 0.393 & 0.765 & \textbf{0.114} & 0.319 & 0.756 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & \textbf{0.182} & \textbf{0.182} & \textbf{0.180} & 0.280 & 0.314 & 0.189 & \textbf{0.186} & \textbf{0.218} & \textbf{0.184} & \textbf{0.308} & 0.127 & 0.217 & \textbf{0.413} \\ 
  ARGOX & 0.188 & 0.186 & 0.182 & \textbf{0.275} & \textbf{0.311} & \textbf{0.183} & 0.197 & 0.231 & 0.200 & 0.338 & 0.122 & \textbf{0.212} & 0.459 \\ 
  VAR1 & 1.330 & 1.175 & 0.888 & 1.792 & 1.926 & 1.814 & 1.755 & 1.609 & 0.829 & 1.959 & 0.382 & 0.576 & 2.074 \\ 
  GFT & -- & -- & -- & 0.604 & 0.633 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.251 & 0.241 & 0.223 & 0.287 & 0.318 & 0.221 & 0.268 & 0.406 & 0.285 & 0.579 & \textbf{0.091} & 0.223 & 0.613 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & \textbf{ 0.979} & \textbf{ 0.979} & \textbf{ 0.978} &  0.938 &  0.925 &  0.954 & \textbf{ 0.976} & \textbf{ 0.983} & \textbf{ 0.953} & \textbf{ 0.977} &  0.910 &  0.922 & \textbf{ 0.943} \\ 
  ARGOX &  0.978 &  0.978 &  0.977 &  0.939 &  0.924 & \textbf{ 0.956} &  0.972 &  0.980 &  0.950 &  0.972 & \textbf{ 0.920} & \textbf{ 0.928} &  0.929 \\ 
  VAR1 &  0.750 &  0.541 &  0.501 &  0.195 & -0.003 &  0.588 &  0.913 &  0.860 &  0.818 &  0.844 &  0.726 &  0.485 &  0.349 \\ 
  GFT & -- & -- & -- & \textbf{ 0.945} & \textbf{ 0.937} & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive &  0.959 &  0.960 &  0.962 &  0.931 &  0.914 &  0.939 &  0.936 &  0.937 &  0.889 &  0.922 &  0.920 &  0.895 &  0.892 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in Illinois.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.IL}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & \textbf{0.544} & \textbf{0.512} & \textbf{0.446} & 0.656 & 0.714 & \textbf{0.416} & 0.718 & \textbf{0.571} & \textbf{0.596} & \textbf{0.810} & 0.163 & 0.230 & \textbf{0.690} \\ 
  ARGOX & 0.566 & 0.537 & 0.478 & 0.714 & 0.778 & 0.431 & \textbf{0.713} & 0.640 & 0.613 & 0.884 & 0.165 & \textbf{0.207} & 0.728 \\ 
  VAR1 & 1.770 & 1.584 & 1.162 & 1.788 & 1.936 & 0.968 & 1.866 & 2.985 & 1.888 & 2.675 & 0.172 & 0.633 & 2.147 \\ 
  GFT & -- & -- & -- & \textbf{0.478} & \textbf{0.521} & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.728 & 0.654 & 0.486 & 0.916 & 1.004 & 0.562 & 0.830 & 0.978 & 0.783 & 1.018 & \textbf{0.103} & 0.248 & 0.863 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & \textbf{0.370} & \textbf{0.333} & \textbf{0.264} & 0.422 & 0.464 & \textbf{0.299} & 0.508 & \textbf{0.412} & 0.430 & 0.540 & 0.126 & 0.157 & \textbf{0.523} \\ 
  ARGOX & 0.377 & 0.339 & 0.268 & 0.465 & 0.518 & 0.303 & \textbf{0.499} & 0.459 & \textbf{0.428} & \textbf{0.516} & 0.133 & \textbf{0.144} & 0.564 \\ 
  VAR1 & 1.240 & 1.057 & 0.717 & 1.341 & 1.494 & 0.727 & 1.294 & 2.375 & 1.547 & 2.281 & 0.131 & 0.481 & 1.727 \\ 
  GFT & -- & -- & -- & \textbf{0.379} & \textbf{0.429} & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.457 & 0.397 & 0.285 & 0.525 & 0.607 & 0.433 & 0.596 & 0.624 & 0.540 & 0.664 & \textbf{0.080} & 0.193 & 0.675 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & \textbf{ 0.951} & \textbf{ 0.948} & \textbf{ 0.936} &  0.937 &  0.931 & \textbf{ 0.870} &  0.896 & \textbf{ 0.974} & \textbf{ 0.915} & \textbf{ 0.927} &  0.911 & \textbf{ 0.963} & \textbf{ 0.939} \\ 
  ARGOX &  0.947 &  0.943 &  0.928 &  0.923 &  0.915 &  0.860 & \textbf{ 0.898} &  0.967 &  0.909 &  0.913 &  0.922 &  0.957 &  0.929 \\ 
  VAR1 &  0.515 &  0.505 &  0.663 &  0.511 &  0.444 &  0.447 &  0.604 &  0.878 &  0.667 & -0.235 &  0.878 &  0.189 &  0.771 \\ 
  GFT & -- & -- & -- & \textbf{ 0.970} & \textbf{ 0.968} & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive &  0.914 &  0.917 &  0.926 &  0.877 &  0.864 &  0.776 &  0.865 &  0.923 &  0.857 &  0.873 & \textbf{ 0.934} &  0.913 &  0.901 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in Indiana.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.IN}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & 0.399 & \textbf{0.686} & \textbf{1.023} & 0.668 & 0.735 & 0.280 & \textbf{0.362} & 0.394 & 0.409 & \textbf{0.537} & 0.930 & \textbf{0.534} & \textbf{1.034} \\ 
  ARGOX & \textbf{0.397} & 0.699 & 1.050 & 0.652 & 0.718 & \textbf{0.267} & 0.388 & \textbf{0.386} & \textbf{0.408} & 0.632 & 0.923 & 0.597 & 1.119 \\ 
  VAR1 & 1.442 & 1.466 & 1.510 & 1.982 & 2.101 & 1.811 & 1.730 & 1.630 & 0.869 & 2.133 & \textbf{0.915} & 0.985 & 1.368 \\ 
  GFT & -- & -- & -- & 2.296 & 2.519 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.463 & 0.786 & 1.169 & \textbf{0.646} & \textbf{0.711} & 0.294 & 0.425 & 0.554 & 0.478 & 0.749 & 0.995 & 0.608 & 1.386 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & 0.244 & \textbf{0.319} & \textbf{0.457} & 0.355 & 0.420 & 0.236 & \textbf{0.260} & 0.304 & \textbf{0.288} & \textbf{0.362} & 0.537 & \textbf{0.383} & \textbf{0.756} \\ 
  ARGOX & \textbf{0.240} & 0.324 & 0.479 & 0.347 & 0.414 & \textbf{0.223} & 0.273 & \textbf{0.285} & 0.298 & 0.396 & 0.546 & 0.426 & 0.802 \\ 
  VAR1 & 1.206 & 1.109 & 0.928 & 1.643 & 1.721 & 1.740 & 1.577 & 1.348 & 0.755 & 1.834 & 0.463 & 0.795 & 1.110 \\ 
  GFT & -- & -- & -- & 1.346 & 1.534 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.261 & 0.350 & 0.514 & \textbf{0.314} & \textbf{0.377} & 0.244 & 0.302 & 0.366 & 0.347 & 0.466 & \textbf{0.419} & 0.429 & 1.041 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & 0.917 & \textbf{0.845} & \textbf{0.759} & 0.677 & 0.600 & 0.706 & \textbf{0.907} & 0.939 & \textbf{0.925} & \textbf{0.926} & 0.495 & \textbf{0.833} & \textbf{0.880} \\ 
  ARGOX & \textbf{0.918} & 0.838 & 0.745 & 0.683 & 0.606 & 0.731 & 0.892 & \textbf{0.940} & 0.924 & 0.902 & 0.508 & 0.791 & 0.854 \\ 
  VAR1 & 0.790 & 0.592 & 0.502 & 0.396 & 0.261 & \textbf{0.802} & 0.710 & 0.886 & 0.821 & 0.781 & 0.488 & 0.379 & 0.835 \\ 
  GFT & -- & -- & -- & 0.575 & 0.507 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.891 & 0.811 & 0.725 & \textbf{0.723} & \textbf{0.668} & 0.702 & 0.875 & 0.878 & 0.895 & 0.852 & \textbf{0.516} & 0.796 & 0.784 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in Iowa.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.IA}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & \textbf{0.523} & \textbf{0.508} & \textbf{0.478} & \textbf{0.702} & \textbf{0.770} & 0.283 & \textbf{0.864} & 0.533 & 0.507 & \textbf{0.635} & 0.212 & 0.482 & \textbf{0.931} \\ 
  ARGOX & 0.526 & 0.515 & 0.494 & 0.729 & 0.799 & \textbf{0.277} & 0.902 & \textbf{0.481} & \textbf{0.456} & 0.668 & 0.213 & 0.472 & 1.012 \\ 
  VAR1 & 1.444 & 1.251 & 0.774 & 1.783 & 1.958 & 0.470 & 2.102 & 2.230 & 0.877 & 1.951 & 0.249 & 0.614 & 1.280 \\ 
  GFT & -- & -- & -- & 1.472 & 1.620 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.678 & 0.633 & 0.542 & 0.898 & 0.986 & 0.298 & 0.971 & 1.021 & 0.554 & 0.874 & \textbf{0.196} & \textbf{0.441} & 1.151 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & 0.332 & 0.322 & \textbf{0.303} & 0.420 & 0.487 & 0.230 & \textbf{0.569} & 0.402 & 0.320 & \textbf{0.503} & 0.157 & 0.352 & \textbf{0.623} \\ 
  ARGOX & \textbf{0.328} & \textbf{0.320} & 0.305 & \textbf{0.412} & \textbf{0.475} & 0.229 & 0.590 & \textbf{0.361} & \textbf{0.307} & 0.516 & 0.157 & 0.349 & 0.676 \\ 
  VAR1 & 0.879 & 0.751 & 0.513 & 1.168 & 1.366 & 0.350 & 1.201 & 1.638 & 0.643 & 1.542 & 0.220 & 0.459 & 0.925 \\ 
  GFT & -- & -- & -- & 1.090 & 1.302 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.404 & 0.376 & 0.326 & 0.528 & 0.614 & \textbf{0.222} & 0.674 & 0.723 & 0.381 & 0.649 & \textbf{0.142} & \textbf{0.323} & 0.860 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & \textbf{0.979} & \textbf{0.974} & \textbf{0.942} & \textbf{0.964} & 0.956 & 0.884 & \textbf{0.944} & 0.990 & 0.949 & \textbf{0.970} & 0.892 & \textbf{0.788} & \textbf{0.903} \\ 
  ARGOX & 0.979 & 0.973 & 0.939 & 0.962 & 0.953 & \textbf{0.890} & 0.939 & \textbf{0.992} & \textbf{0.960} & 0.968 & 0.891 & 0.778 & 0.882 \\ 
  VAR1 & 0.883 & 0.863 & 0.845 & 0.860 & 0.845 & 0.764 & 0.758 & 0.957 & 0.836 & 0.909 & \textbf{0.923} & 0.688 & 0.814 \\ 
  GFT & -- & -- & -- & 0.960 & \textbf{0.957} & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.964 & 0.960 & 0.931 & 0.939 & 0.924 & 0.874 & 0.929 & 0.964 & 0.937 & 0.943 & 0.899 & 0.785 & 0.850 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in Kansas.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.KS}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & \textbf{0.670} & \textbf{0.631} & \textbf{0.550} & \textbf{0.279} & \textbf{0.306} & 0.254 & \textbf{1.071} & 1.018 & \textbf{0.837} & \textbf{0.997} & 0.215 & 0.391 & \textbf{1.210} \\ 
  ARGOX & 0.683 & 0.656 & 0.603 & 0.293 & 0.322 & \textbf{0.244} & 1.075 & \textbf{0.996} & 0.875 & 1.163 & 0.217 & \textbf{0.347} & 1.280 \\ 
  VAR1 & 1.698 & 1.507 & 1.067 & 2.646 & 2.906 & 0.741 & 1.284 & 1.900 & 2.522 & 2.259 & 0.275 & 0.636 & 2.434 \\ 
  GFT & -- & -- & -- & 2.912 & 3.180 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.850 & 0.774 & 0.607 & 0.393 & 0.432 & 0.281 & 1.222 & 1.300 & 1.038 & 1.384 & \textbf{0.174} & 0.395 & 1.438 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & \textbf{0.379} & \textbf{0.353} & 0.306 & \textbf{0.178} & \textbf{0.206} & 0.164 & \textbf{0.798} & 0.692 & \textbf{0.504} & \textbf{0.658} & 0.168 & 0.306 & \textbf{0.860} \\ 
  ARGOX & 0.391 & 0.361 & \textbf{0.306} & 0.188 & 0.216 & \textbf{0.158} & 0.830 & \textbf{0.668} & 0.533 & 0.746 & 0.171 & \textbf{0.261} & 0.907 \\ 
  VAR1 & 1.019 & 0.869 & 0.590 & 2.027 & 2.365 & 0.697 & 0.834 & 1.229 & 1.544 & 1.768 & 0.235 & 0.464 & 1.738 \\ 
  GFT & -- & -- & -- & 2.101 & 2.363 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.465 & 0.420 & 0.337 & 0.220 & 0.265 & 0.190 & 0.913 & 0.871 & 0.680 & 0.975 & \textbf{0.136} & 0.324 & 1.099 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & \textbf{0.971} & \textbf{0.968} & \textbf{0.953} & 0.952 & 0.947 & 0.925 & \textbf{0.925} & 0.965 & \textbf{0.957} & \textbf{0.955} & 0.848 & 0.921 & \textbf{0.903} \\ 
  ARGOX & 0.970 & 0.965 & 0.945 & 0.946 & 0.941 & \textbf{0.931} & 0.924 & \textbf{0.968} & 0.953 & 0.940 & 0.860 & \textbf{0.923} & 0.889 \\ 
  VAR1 & 0.797 & 0.797 & 0.800 & 0.777 & 0.749 & 0.916 & 0.894 & 0.872 & 0.723 & 0.772 & 0.808 & 0.728 & 0.657 \\ 
  GFT & -- & -- & -- & \textbf{0.962} & \textbf{0.959} & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.954 & 0.952 & 0.943 & 0.906 & 0.895 & 0.908 & 0.898 & 0.941 & 0.934 & 0.909 & \textbf{0.862} & 0.859 & 0.867 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in Kentucky.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.KY}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & \textbf{0.511} & \textbf{0.487} & 0.438 & 0.488 & 0.534 & 0.276 & \textbf{0.274} & \textbf{0.617} & 0.870 & \textbf{0.896} & 0.507 & 0.350 & \textbf{0.569} \\ 
  ARGOX & 0.524 & 0.496 & \textbf{0.438} & \textbf{0.455} & \textbf{0.498} & 0.264 & 0.277 & 0.679 & \textbf{0.866} & 0.937 & 0.491 & \textbf{0.317} & 0.655 \\ 
  VAR1 & 2.297 & 2.099 & 1.671 & 2.946 & 3.199 & 1.567 & 2.045 & 2.380 & 1.876 & 4.363 & 0.345 & 0.769 & 2.875 \\ 
  GFT & -- & -- & -- & 1.015 & 1.106 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.641 & 0.612 & 0.553 & 0.567 & 0.621 & \textbf{0.249} & 0.355 & 0.917 & 0.981 & 1.373 & \textbf{0.323} & 0.385 & 0.680 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & \textbf{0.306} & \textbf{0.299} & \textbf{0.287} & 0.325 & 0.371 & 0.230 & \textbf{0.200} & \textbf{0.429} & \textbf{0.491} & \textbf{0.682} & 0.318 & 0.225 & \textbf{0.471} \\ 
  ARGOX & 0.318 & 0.308 & 0.290 & \textbf{0.310} & \textbf{0.355} & 0.220 & 0.215 & 0.476 & 0.515 & 0.741 & 0.303 & \textbf{0.198} & 0.562 \\ 
  VAR1 & 1.888 & 1.599 & 1.065 & 2.661 & 2.979 & 1.501 & 1.598 & 2.032 & 1.666 & 3.708 & 0.289 & 0.686 & 2.146 \\ 
  GFT & -- & -- & -- & 0.748 & 0.838 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.386 & 0.361 & 0.315 & 0.384 & 0.441 & \textbf{0.195} & 0.272 & 0.608 & 0.705 & 1.121 & \textbf{0.144} & 0.267 & 0.592 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & \textbf{0.979} & \textbf{0.980} & 0.976 & 0.964 & 0.952 & 0.871 & \textbf{0.968} & \textbf{0.980} & \textbf{0.951} & \textbf{0.952} & 0.252 & \textbf{0.955} & \textbf{0.898} \\ 
  ARGOX & 0.978 & 0.979 & \textbf{0.976} & 0.968 & 0.955 & \textbf{0.878} & 0.968 & 0.976 & 0.950 & 0.948 & 0.244 & 0.951 & 0.866 \\ 
  VAR1 & 0.769 & 0.711 & 0.621 & 0.735 & 0.708 & 0.725 & 0.714 & 0.774 & 0.906 & 0.659 & \textbf{0.442} & 0.775 & 0.408 \\ 
  GFT & -- & -- & -- & \textbf{0.981} & \textbf{0.978} & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.968 & 0.968 & 0.965 & 0.946 & 0.924 & 0.876 & 0.948 & 0.952 & 0.927 & 0.884 & 0.422 & 0.878 & 0.849 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in Louisiana.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.LA}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & \textbf{0.276} & \textbf{0.391} & \textbf{0.542} & \textbf{0.327} & \textbf{0.352} & 0.335 & \textbf{0.274} & \textbf{0.248} & \textbf{0.293} & \textbf{0.828} & 0.127 & 0.287 & \textbf{1.136} \\ 
  ARGOX & 0.278 & 0.398 & 0.556 & 0.328 & 0.353 & \textbf{0.332} & 0.280 & 0.251 & 0.296 & 0.857 & 0.117 & 0.317 & 1.142 \\ 
  VAR1 & 3.012 & 2.731 & 2.112 & 2.174 & 2.376 & 1.319 & 2.017 & 5.069 & 3.685 & 5.899 & 0.617 & 0.840 & 2.727 \\ 
  GFT & -- & -- & -- & 0.744 & 0.813 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.296 & 0.428 & 0.602 & 0.354 & 0.380 & 0.375 & 0.297 & 0.253 & 0.297 & 0.865 & \textbf{0.114} & \textbf{0.255} & 1.354 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & \textbf{0.203} & \textbf{0.222} & \textbf{0.257} & 0.253 & 0.273 & 0.269 & \textbf{0.216} & \textbf{0.197} & 0.236 & \textbf{0.440} & 0.099 & 0.218 & \textbf{0.805} \\ 
  ARGOX & 0.204 & 0.224 & 0.262 & \textbf{0.252} & \textbf{0.272} & \textbf{0.266} & 0.220 & 0.197 & 0.238 & 0.453 & 0.093 & 0.230 & 0.811 \\ 
  VAR1 & 2.244 & 1.931 & 1.350 & 1.792 & 2.047 & 1.229 & 1.786 & 4.150 & 3.133 & 5.433 & 0.514 & 0.680 & 2.165 \\ 
  GFT & -- & -- & -- & 0.482 & 0.547 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.216 & 0.238 & 0.278 & 0.273 & 0.292 & 0.290 & 0.229 & 0.208 & \textbf{0.232} & 0.451 & \textbf{0.091} & \textbf{0.193} & 1.034 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & \textbf{0.952} & \textbf{0.944} & \textbf{0.940} & 0.886 & 0.859 & 0.295 & \textbf{0.804} & \textbf{0.792} & \textbf{0.945} & \textbf{0.894} & 0.693 & 0.878 & 0.921 \\ 
  ARGOX & 0.951 & 0.943 & 0.939 & 0.885 & 0.858 & 0.306 & 0.793 & 0.787 & 0.943 & 0.887 & \textbf{0.702} & 0.856 & \textbf{0.921} \\ 
  VAR1 & 0.677 & 0.534 & 0.506 & 0.696 & 0.600 & \textbf{0.328} & 0.497 & 0.625 & 0.845 & 0.571 & 0.281 & 0.211 & 0.272 \\ 
  GFT & -- & -- & -- & \textbf{0.917} & \textbf{0.916} & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.945 & 0.933 & 0.926 & 0.871 & 0.844 & 0.257 & 0.789 & 0.760 & 0.940 & 0.885 & 0.645 & \textbf{0.897} & 0.882 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in Maine.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.ME}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & \textbf{0.479} & \textbf{0.462} & \textbf{0.431} & \textbf{0.540} & \textbf{0.514} & \textbf{0.568} & \textbf{0.593} & 0.446 & 0.511 & 0.646 & 0.135 & \textbf{0.428} & \textbf{0.791} \\ 
  ARGOX & 0.494 & 0.476 & 0.440 & 0.558 & 0.522 & 0.580 & 0.621 & \textbf{0.438} & \textbf{0.510} & \textbf{0.639} & \textbf{0.126} & 0.459 & 0.893 \\ 
  VAR1 & 1.055 & 1.168 & 1.352 & 1.089 & 1.098 & 1.237 & 1.329 & 0.993 & 0.775 & 1.705 & 0.417 & 0.806 & 3.443 \\ 
  GFT & -- & -- & -- & 1.282 & 1.387 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.601 & 0.565 & 0.491 & 0.714 & 0.743 & 0.657 & 0.721 & 0.619 & 0.624 & 0.810 & 0.134 & 0.564 & 0.893 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & \textbf{0.353} & \textbf{0.318} & \textbf{0.253} & 0.364 & 0.326 & \textbf{0.440} & \textbf{0.463} & \textbf{0.336} & 0.403 & \textbf{0.451} & 0.108 & \textbf{0.278} & \textbf{0.638} \\ 
  ARGOX & 0.362 & 0.327 & 0.262 & \textbf{0.359} & \textbf{0.311} & 0.450 & 0.492 & 0.348 & \textbf{0.402} & 0.498 & \textbf{0.103} & 0.280 & 0.745 \\ 
  VAR1 & 0.768 & 0.791 & 0.832 & 0.730 & 0.674 & 0.990 & 0.939 & 0.672 & 0.640 & 1.279 & 0.377 & 0.642 & 3.007 \\ 
  GFT & -- & -- & -- & 1.023 & 1.137 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.416 & 0.371 & 0.289 & 0.447 & 0.434 & 0.494 & 0.510 & 0.444 & 0.496 & 0.620 & 0.106 & 0.335 & 0.743 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & \textbf{ 0.942} & \textbf{ 0.950} & \textbf{ 0.962} & \textbf{ 0.859} &  0.894 & \textbf{ 0.745} & \textbf{ 0.924} &  0.963 &  0.914 &  0.956 &  0.916 & \textbf{ 0.924} & \textbf{ 0.900} \\ 
  ARGOX &  0.939 &  0.947 &  0.960 &  0.841 &  0.884 &  0.730 &  0.913 & \textbf{ 0.964} & \textbf{ 0.915} & \textbf{ 0.957} & \textbf{ 0.920} &  0.905 &  0.875 \\ 
  VAR1 &  0.765 &  0.714 &  0.687 &  0.358 &  0.396 &  0.223 &  0.849 &  0.794 &  0.814 &  0.789 &  0.824 &  0.694 & -0.081 \\ 
  GFT & -- & -- & -- &  0.853 & \textbf{ 0.926} & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive &  0.911 &  0.928 &  0.952 &  0.753 &  0.775 &  0.695 &  0.872 &  0.924 &  0.876 &  0.918 &  0.905 &  0.838 &  0.869 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in Maryland.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.MD}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & \textbf{0.242} & \textbf{0.326} & \textbf{0.442} & 0.275 & \textbf{0.296} & 0.230 & \textbf{0.190} & \textbf{0.369} & \textbf{0.188} & 0.621 & 0.115 & \textbf{0.426} & \textbf{0.897} \\ 
  ARGOX & 0.249 & 0.331 & 0.446 & \textbf{0.275} & 0.297 & \textbf{0.223} & 0.204 & 0.381 & 0.213 & \textbf{0.619} & 0.101 & 0.445 & 0.911 \\ 
  VAR1 & 0.720 & 0.864 & 1.080 & 0.648 & 0.621 & 0.816 & 0.892 & 0.419 & 0.652 & 1.012 & 0.415 & 0.920 & 2.514 \\ 
  GFT & -- & -- & -- & 0.344 & 0.353 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.329 & 0.415 & 0.540 & 0.335 & 0.363 & 0.258 & 0.271 & 0.541 & 0.324 & 0.711 & \textbf{0.085} & 0.500 & 1.229 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & \textbf{0.161} & \textbf{0.188} & \textbf{0.239} & 0.186 & 0.196 & 0.171 & \textbf{0.154} & \textbf{0.263} & \textbf{0.146} & \textbf{0.393} & 0.092 & \textbf{0.311} & \textbf{0.604} \\ 
  ARGOX & 0.163 & 0.191 & 0.242 & \textbf{0.177} & \textbf{0.189} & \textbf{0.163} & 0.159 & 0.276 & 0.162 & 0.404 & 0.079 & 0.326 & 0.635 \\ 
  VAR1 & 0.577 & 0.638 & 0.752 & 0.506 & 0.461 & 0.681 & 0.653 & 0.316 & 0.540 & 0.835 & 0.386 & 0.756 & 1.997 \\ 
  GFT & -- & -- & -- & 0.266 & 0.260 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.208 & 0.234 & 0.282 & 0.237 & 0.258 & 0.181 & 0.203 & 0.368 & 0.231 & 0.550 & \textbf{0.061} & 0.376 & 0.861 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & \textbf{0.975} & \textbf{0.970} & \textbf{0.966} & 0.916 & 0.908 & 0.888 & \textbf{0.954} & \textbf{0.965} & \textbf{0.973} & 0.936 & 0.918 & \textbf{0.922} & \textbf{0.952} \\ 
  ARGOX & 0.973 & 0.969 & 0.965 & 0.920 & 0.913 & \textbf{0.894} & 0.947 & 0.963 & 0.964 & 0.938 & 0.923 & 0.913 & 0.948 \\ 
  VAR1 & 0.846 & 0.824 & 0.806 & 0.534 & 0.571 & 0.533 & 0.819 & 0.950 & 0.801 & \textbf{0.943} & 0.879 & 0.590 & 0.426 \\ 
  GFT & -- & -- & -- & \textbf{0.940} & \textbf{0.931} & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.952 & 0.949 & 0.946 & 0.877 & 0.861 & 0.870 & 0.908 & 0.919 & 0.919 & 0.912 & \textbf{0.927} & 0.890 & 0.892 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in Massachusetts.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.MA}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & 0.276 & \textbf{0.250} & \textbf{0.194} & \textbf{0.366} & \textbf{0.398} & 0.207 & 0.332 & 0.338 & 0.298 & \textbf{0.316} & 0.132 & \textbf{0.223} & 0.329 \\ 
  ARGOX & \textbf{0.275} & 0.252 & 0.201 & 0.384 & 0.419 & \textbf{0.199} & \textbf{0.328} & \textbf{0.319} & \textbf{0.285} & 0.344 & \textbf{0.130} & 0.238 & \textbf{0.326} \\ 
  VAR1 & 1.020 & 1.029 & 1.046 & 0.980 & 1.048 & 0.646 & 1.471 & 2.000 & 0.605 & 1.188 & 0.173 & 0.408 & 2.644 \\ 
  GFT & -- & -- & -- & 1.203 & 1.302 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.359 & 0.329 & 0.266 & 0.538 & 0.591 & 0.257 & 0.411 & 0.489 & 0.329 & 0.437 & 0.132 & 0.245 & 0.520 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & \textbf{0.193} & \textbf{0.173} & \textbf{0.137} & \textbf{0.247} & \textbf{0.278} & 0.165 & \textbf{0.226} & 0.273 & 0.226 & \textbf{0.230} & 0.106 & \textbf{0.163} & 0.255 \\ 
  ARGOX & 0.194 & 0.175 & 0.140 & 0.264 & 0.302 & \textbf{0.158} & 0.238 & \textbf{0.248} & \textbf{0.221} & 0.259 & 0.108 & 0.171 & \textbf{0.253} \\ 
  VAR1 & 0.673 & 0.610 & 0.493 & 0.741 & 0.783 & 0.447 & 1.138 & 1.582 & 0.501 & 0.760 & 0.146 & 0.331 & 1.845 \\ 
  GFT & -- & -- & -- & 1.017 & 1.126 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.234 & 0.212 & 0.171 & 0.304 & 0.353 & 0.184 & 0.299 & 0.403 & 0.255 & 0.321 & \textbf{0.103} & 0.176 & 0.412 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & 0.967 & \textbf{0.969} & \textbf{0.972} & 0.939 & 0.931 & 0.950 & 0.947 & 0.973 & 0.861 & \textbf{0.962} & 0.238 & \textbf{0.855} & 0.939 \\ 
  ARGOX & \textbf{0.967} & 0.969 & 0.971 & 0.932 & 0.925 & \textbf{0.957} & \textbf{0.949} & \textbf{0.977} & \textbf{0.875} & 0.954 & 0.254 & 0.835 & \textbf{0.940} \\ 
  VAR1 & 0.479 & 0.542 & 0.848 & 0.382 & 0.250 & 0.124 & 0.333 & 0.627 & 0.632 & 0.812 & \textbf{0.389} & 0.620 & 0.816 \\ 
  GFT & -- & -- & -- & \textbf{0.978} & \textbf{0.976} & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.944 & 0.947 & 0.949 & 0.860 & 0.839 & 0.917 & 0.917 & 0.936 & 0.837 & 0.924 & 0.174 & 0.804 & 0.849 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in Michigan.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.MI}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & \textbf{0.571} & \textbf{0.568} & \textbf{0.561} & \textbf{0.611} & \textbf{0.658} & \textbf{0.560} & \textbf{0.415} & 0.407 & \textbf{0.503} & \textbf{1.187} & 0.239 & \textbf{0.963} & \textbf{0.666} \\ 
  ARGOX & 0.578 & 0.593 & 0.619 & 0.653 & 0.706 & 0.565 & 0.420 & \textbf{0.375} & 0.505 & 1.248 & 0.253 & 1.016 & 0.768 \\ 
  VAR1 & 1.153 & 1.164 & 1.185 & 1.557 & 1.693 & 0.758 & 0.812 & 0.934 & 1.185 & 2.129 & 0.198 & 2.103 & 1.641 \\ 
  GFT & -- & -- & -- & 0.780 & 0.850 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.721 & 0.671 & 0.567 & 0.898 & 0.970 & 0.714 & 0.526 & 0.502 & 0.538 & 1.437 & \textbf{0.092} & 0.984 & 0.770 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & \textbf{0.362} & \textbf{0.342} & 0.306 & \textbf{0.417} & \textbf{0.454} & 0.476 & \textbf{0.318} & 0.330 & \textbf{0.363} & \textbf{0.654} & 0.182 & 0.575 & \textbf{0.438} \\ 
  ARGOX & 0.365 & 0.356 & 0.339 & 0.455 & 0.498 & \textbf{0.475} & 0.331 & \textbf{0.310} & 0.364 & 0.678 & 0.202 & 0.626 & 0.548 \\ 
  VAR1 & 0.816 & 0.764 & 0.666 & 1.156 & 1.283 & 0.565 & 0.681 & 0.757 & 1.002 & 1.679 & 0.149 & 1.509 & 1.275 \\ 
  GFT & -- & -- & -- & 0.573 & 0.653 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.431 & 0.375 & \textbf{0.271} & 0.584 & 0.641 & 0.544 & 0.378 & 0.392 & 0.402 & 0.775 & \textbf{0.076} & \textbf{0.475} & 0.563 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & \textbf{0.924} & \textbf{0.926} & 0.924 & \textbf{0.928} & \textbf{0.919} & \textbf{0.741} & \textbf{0.936} & 0.976 & \textbf{0.835} & \textbf{0.786} & 0.665 & 0.827 & \textbf{0.901} \\ 
  ARGOX & 0.922 & 0.919 & 0.908 & 0.917 & 0.905 & 0.734 & 0.936 & \textbf{0.979} & 0.835 & 0.760 & 0.688 & 0.806 & 0.869 \\ 
  VAR1 & 0.814 & 0.786 & 0.704 & 0.791 & 0.755 & 0.689 & 0.768 & 0.957 & 0.500 & 0.684 & 0.055 & 0.532 & 0.241 \\ 
  GFT & -- & -- & -- & 0.927 & 0.916 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.882 & 0.900 & \textbf{0.926} & 0.844 & 0.825 & 0.629 & 0.888 & 0.959 & 0.807 & 0.670 & \textbf{0.864} & \textbf{0.829} & 0.861 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in Minnesota.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.MN}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & \textbf{0.568} & \textbf{0.561} & \textbf{0.547} & \textbf{0.652} & \textbf{0.713} & \textbf{0.353} & \textbf{0.486} & \textbf{0.939} & \textbf{0.632} & \textbf{0.691} & \textbf{0.400} & \textbf{0.428} & \textbf{1.131} \\ 
  ARGOX & 0.610 & 0.604 & 0.591 & 0.755 & 0.828 & 0.354 & 0.488 & 1.027 & 0.636 & 0.763 & 0.400 & 0.438 & 1.270 \\ 
  VAR1 & 2.273 & 2.162 & 1.938 & 2.985 & 3.274 & 1.781 & 1.877 & 4.023 & 2.191 & 2.034 & 1.610 & 1.553 & 3.783 \\ 
  GFT & -- & -- & -- & 1.454 & 1.561 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.790 & 0.751 & 0.673 & 1.022 & 1.123 & 0.448 & 0.650 & 1.320 & 0.840 & 0.946 & 0.446 & 0.634 & 1.384 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & \textbf{0.381} & \textbf{0.387} & \textbf{0.398} & \textbf{0.467} & \textbf{0.531} & \textbf{0.285} & \textbf{0.388} & \textbf{0.666} & \textbf{0.411} & \textbf{0.555} & \textbf{0.313} & 0.333 & \textbf{0.983} \\ 
  ARGOX & 0.403 & 0.406 & 0.412 & 0.519 & 0.598 & 0.289 & 0.393 & 0.730 & 0.429 & 0.595 & 0.314 & \textbf{0.316} & 1.115 \\ 
  VAR1 & 1.605 & 1.600 & 1.591 & 2.362 & 2.740 & 1.676 & 1.593 & 2.812 & 1.533 & 1.643 & 1.499 & 1.343 & 3.178 \\ 
  GFT & -- & -- & -- & 1.284 & 1.394 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.507 & 0.495 & 0.473 & 0.665 & 0.781 & 0.344 & 0.519 & 0.906 & 0.601 & 0.769 & 0.354 & 0.442 & 1.178 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & \textbf{ 0.969} & \textbf{ 0.964} & \textbf{ 0.944} & \textbf{ 0.964} & \textbf{ 0.952} &  0.891 &  0.933 & \textbf{ 0.966} & \textbf{ 0.958} & \textbf{ 0.939} &  0.663 & \textbf{ 0.932} & \textbf{ 0.854} \\ 
  ARGOX &  0.964 &  0.958 &  0.935 &  0.951 &  0.935 & \textbf{ 0.891} & \textbf{ 0.933} &  0.960 &  0.957 &  0.926 & \textbf{ 0.663} &  0.931 &  0.820 \\ 
  VAR1 &  0.681 &  0.666 &  0.661 &  0.706 &  0.650 &  0.641 &  0.638 &  0.432 &  0.673 &  0.659 & -0.259 &  0.550 &  0.365 \\ 
  GFT & -- & -- & -- &  0.956 &  0.949 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive &  0.940 &  0.936 &  0.918 &  0.910 &  0.881 &  0.835 &  0.883 &  0.928 &  0.912 &  0.874 &  0.617 &  0.852 &  0.784 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in Mississippi.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.MS}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & \textbf{0.658} & \textbf{0.584} & \textbf{0.410} & \textbf{0.531} & \textbf{0.564} & 0.370 & \textbf{0.624} & 0.949 & \textbf{0.807} & \textbf{1.223} & 0.164 & 0.372 & \textbf{0.553} \\ 
  ARGOX & 0.670 & 0.608 & 0.472 & 0.561 & 0.600 & \textbf{0.360} & 0.676 & \textbf{0.946} & 0.840 & 1.335 & 0.154 & \textbf{0.331} & 0.580 \\ 
  VAR1 & 0.876 & 0.759 & 0.470 & 0.895 & 0.971 & 0.394 & 0.761 & 1.378 & 1.012 & 1.542 & \textbf{0.107} & 0.396 & 0.741 \\ 
  GFT & -- & -- & -- & 0.728 & 0.786 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.843 & 0.744 & 0.511 & 0.911 & 0.989 & 0.393 & 0.692 & 1.368 & 1.008 & 1.474 & 0.112 & 0.406 & 0.726 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & \textbf{0.393} & \textbf{0.348} & 0.264 & \textbf{0.355} & \textbf{0.370} & 0.302 & \textbf{0.410} & 0.614 & \textbf{0.561} & \textbf{0.841} & 0.130 & 0.260 & \textbf{0.407} \\ 
  ARGOX & 0.396 & 0.352 & 0.271 & 0.375 & 0.396 & \textbf{0.284} & 0.455 & \textbf{0.610} & 0.571 & 0.891 & 0.126 & \textbf{0.241} & 0.423 \\ 
  VAR1 & 0.488 & 0.405 & \textbf{0.249} & 0.491 & 0.542 & 0.311 & 0.489 & 0.884 & 0.719 & 1.045 & \textbf{0.084} & 0.259 & 0.553 \\ 
  GFT & -- & -- & -- & 0.604 & 0.670 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.484 & 0.407 & 0.265 & 0.528 & 0.586 & 0.311 & 0.466 & 0.907 & 0.718 & 1.035 & 0.085 & 0.271 & 0.533 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & \textbf{0.960} & \textbf{0.960} & \textbf{0.966} & \textbf{0.961} & 0.953 & 0.771 & \textbf{0.932} & 0.970 & \textbf{0.940} & \textbf{0.929} & 0.845 & 0.961 & \textbf{0.943} \\ 
  ARGOX & 0.959 & 0.957 & 0.958 & 0.957 & 0.947 & \textbf{0.784} & 0.920 & \textbf{0.970} & 0.929 & 0.917 & 0.846 & \textbf{0.961} & 0.934 \\ 
  VAR1 & 0.930 & 0.933 & 0.947 & 0.886 & 0.857 & 0.756 & 0.912 & 0.934 & 0.886 & 0.894 & \textbf{0.908} & 0.926 & 0.894 \\ 
  GFT & -- & -- & -- & 0.959 & \textbf{0.964} & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.934 & 0.936 & 0.946 & 0.886 & 0.858 & 0.761 & 0.919 & 0.936 & 0.890 & 0.900 & 0.904 & 0.919 & 0.896 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in Missouri.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.MO}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & \textbf{0.227} & \textbf{0.284} & \textbf{0.368} & \textbf{0.249} & \textbf{0.271} & 0.233 & \textbf{0.141} & 0.157 & 0.439 & \textbf{0.390} & \textbf{0.166} & \textbf{0.349} & \textbf{0.811} \\ 
  ARGOX & 0.229 & 0.291 & 0.381 & 0.254 & 0.277 & \textbf{0.233} & 0.143 & \textbf{0.157} & 0.440 & 0.398 & 0.167 & 0.362 & 0.850 \\ 
  VAR1 & 3.395 & 2.943 & 1.829 & 4.147 & 4.503 & 2.903 & 3.537 & 6.030 & 2.562 & 2.865 & 1.351 & 1.787 & 3.343 \\ 
  GFT & -- & -- & -- & 1.100 & 1.192 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.241 & 0.317 & 0.424 & 0.296 & 0.323 & 0.259 & 0.154 & 0.174 & \textbf{0.429} & 0.457 & 0.166 & 0.394 & 0.953 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & \textbf{0.136} & \textbf{0.168} & \textbf{0.225} & \textbf{0.181} & \textbf{0.204} & \textbf{0.160} & \textbf{0.097} & 0.117 & \textbf{0.320} & \textbf{0.276} & \textbf{0.123} & \textbf{0.262} & \textbf{0.557} \\ 
  ARGOX & 0.137 & 0.169 & 0.229 & 0.184 & 0.208 & 0.161 & 0.099 & \textbf{0.117} & 0.321 & 0.283 & 0.124 & 0.265 & 0.586 \\ 
  VAR1 & 2.805 & 2.369 & 1.559 & 3.685 & 4.120 & 2.838 & 3.325 & 5.030 & 2.358 & 2.514 & 1.237 & 1.619 & 2.868 \\ 
  GFT & -- & -- & -- & 0.930 & 1.029 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.140 & 0.179 & 0.253 & 0.188 & 0.213 & 0.169 & 0.112 & 0.123 & 0.320 & 0.325 & 0.125 & 0.287 & 0.682 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & \textbf{0.961} & \textbf{0.958} & \textbf{0.942} & 0.898 & 0.887 & 0.421 & \textbf{0.575} & 0.751 & 0.919 & \textbf{0.958} & 0.816 & \textbf{0.818} & \textbf{0.885} \\ 
  ARGOX & 0.960 & 0.956 & 0.939 & 0.893 & 0.881 & 0.412 & 0.562 & \textbf{0.753} & 0.919 & 0.956 & 0.816 & 0.808 & 0.875 \\ 
  VAR1 & 0.497 & 0.460 & 0.735 & 0.703 & 0.655 & \textbf{0.689} & 0.276 & 0.357 & \textbf{0.945} & 0.639 & 0.087 & 0.659 & 0.332 \\ 
  GFT & -- & -- & -- & \textbf{0.938} & \textbf{0.930} & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.956 & 0.948 & 0.925 & 0.861 & 0.845 & 0.341 & 0.499 & 0.725 & 0.916 & 0.942 & \textbf{0.823} & 0.766 & 0.852 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in Montana.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.MT}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & \textbf{0.605} & \textbf{0.600} & \textbf{0.591} & \textbf{0.698} & \textbf{0.766} & 0.326 & \textbf{0.466} & 0.823 & \textbf{0.828} & \textbf{0.789} & 0.239 & \textbf{0.362} & \textbf{1.489} \\ 
  ARGOX & 0.617 & 0.617 & 0.617 & 0.707 & 0.777 & 0.303 & 0.492 & \textbf{0.817} & 0.894 & 0.850 & 0.230 & 0.389 & 1.536 \\ 
  VAR1 & 2.160 & 1.991 & 1.632 & 1.568 & 1.711 & 0.491 & 1.314 & 3.915 & 3.141 & 2.887 & 0.415 & 1.269 & 4.152 \\ 
  GFT & -- & -- & -- & 0.866 & 0.951 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.704 & 0.702 & 0.697 & 0.835 & 0.918 & \textbf{0.286} & 0.521 & 0.913 & 0.972 & 1.100 & \textbf{0.193} & 0.479 & 1.744 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & 0.388 & \textbf{0.377} & \textbf{0.357} & 0.401 & 0.464 & 0.259 & \textbf{0.330} & 0.606 & \textbf{0.538} & \textbf{0.575} & 0.203 & \textbf{0.285} & \textbf{1.091} \\ 
  ARGOX & \textbf{0.388} & 0.382 & 0.371 & \textbf{0.397} & \textbf{0.461} & 0.242 & 0.343 & \textbf{0.595} & 0.583 & 0.623 & 0.195 & 0.295 & 1.162 \\ 
  VAR1 & 1.435 & 1.287 & 1.013 & 1.206 & 1.356 & 0.403 & 0.951 & 3.412 & 2.361 & 2.144 & 0.353 & 1.121 & 3.299 \\ 
  GFT & -- & -- & -- & 0.530 & 0.618 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.433 & 0.417 & 0.387 & 0.479 & 0.564 & \textbf{0.211} & 0.353 & 0.693 & 0.684 & 0.692 & \textbf{0.160} & 0.338 & 1.336 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & \textbf{0.950} & \textbf{0.951} & \textbf{0.952} & 0.840 & 0.812 & 0.536 & \textbf{0.883} & 0.927 & \textbf{0.927} & \textbf{0.942} & 0.607 & \textbf{0.878} & \textbf{0.892} \\ 
  ARGOX & 0.948 & 0.948 & 0.947 & 0.838 & 0.810 & 0.591 & 0.870 & \textbf{0.929} & 0.913 & 0.936 & 0.628 & 0.850 & 0.881 \\ 
  VAR1 & 0.589 & 0.623 & 0.751 & 0.807 & 0.776 & 0.380 & 0.660 & 0.662 & 0.256 & 0.381 & 0.462 & 0.434 & 0.577 \\ 
  GFT & -- & -- & -- & \textbf{0.842} & \textbf{0.816} & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.934 & 0.935 & 0.934 & 0.785 & 0.752 & \textbf{0.608} & 0.859 & 0.900 & 0.901 & 0.872 & \textbf{0.674} & 0.765 & 0.846 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in Nebraska.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.NE}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & \textbf{0.308} & \textbf{0.333} & \textbf{0.374} & \textbf{0.365} & \textbf{0.400} & 0.332 & \textbf{0.245} & \textbf{0.215} & \textbf{0.368} & 0.518 & 0.403 & \textbf{0.319} & \textbf{0.370} \\ 
  ARGOX & 0.310 & 0.338 & 0.384 & 0.371 & 0.406 & \textbf{0.332} & 0.254 & 0.221 & 0.369 & 0.527 & \textbf{0.400} & 0.321 & 0.430 \\ 
  VAR1 & 1.351 & 1.313 & 1.240 & 0.557 & 0.580 & 1.095 & 2.185 & 2.248 & 1.059 & 1.985 & 0.479 & 0.887 & 2.850 \\ 
  GFT & -- & -- & -- & 1.658 & 1.705 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.330 & 0.359 & 0.408 & 0.447 & 0.489 & 0.363 & 0.245 & 0.354 & 0.429 & \textbf{0.394} & 0.418 & 0.354 & 0.550 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & \textbf{0.209} & \textbf{0.236} & \textbf{0.285} & \textbf{0.272} & \textbf{0.315} & \textbf{0.235} & 0.187 & \textbf{0.174} & 0.231 & 0.418 & 0.303 & 0.238 & \textbf{0.294} \\ 
  ARGOX & 0.210 & 0.237 & 0.288 & 0.278 & 0.321 & 0.240 & 0.195 & 0.175 & \textbf{0.230} & 0.424 & \textbf{0.298} & \textbf{0.230} & 0.325 \\ 
  VAR1 & 0.830 & 0.820 & 0.800 & 0.447 & 0.454 & 0.921 & 1.507 & 1.457 & 0.759 & 1.626 & 0.389 & 0.777 & 2.361 \\ 
  GFT & -- & -- & -- & 1.569 & 1.602 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.220 & 0.248 & 0.300 & 0.310 & 0.356 & 0.251 & \textbf{0.185} & 0.270 & 0.283 & \textbf{0.320} & 0.316 & 0.265 & 0.423 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & \textbf{0.940} & \textbf{0.931} & \textbf{0.902} & 0.950 & 0.941 & \textbf{0.886} & \textbf{0.885} & \textbf{0.976} & \textbf{0.923} & 0.809 & \textbf{0.700} & \textbf{0.860} & \textbf{0.939} \\ 
  ARGOX & 0.939 & 0.929 & 0.897 & \textbf{0.950} & \textbf{0.942} & 0.886 & 0.872 & 0.975 & 0.922 & 0.803 & 0.700 & 0.860 & 0.919 \\ 
  VAR1 & 0.618 & 0.549 & 0.492 & 0.909 & 0.891 & 0.655 & 0.281 & 0.618 & 0.769 & 0.057 & 0.679 & 0.787 & 0.635 \\ 
  GFT & -- & -- & -- & 0.930 & 0.919 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.932 & 0.922 & 0.888 & 0.922 & 0.909 & 0.859 & 0.865 & 0.930 & 0.898 & \textbf{0.866} & 0.696 & 0.827 & 0.862 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in Nevada.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.NV}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & 0.407 & \textbf{0.407} & 0.406 & 0.285 & 0.312 & 0.152 & 0.340 & \textbf{0.719} & 0.605 & 0.662 & \textbf{0.230} & 0.584 & \textbf{0.269} \\ 
  ARGOX & \textbf{0.406} & 0.411 & 0.421 & 0.272 & 0.298 & \textbf{0.148} & \textbf{0.327} & 0.727 & \textbf{0.595} & 0.709 & 0.236 & \textbf{0.581} & 0.284 \\ 
  VAR1 & 0.872 & 1.390 & 2.027 & 1.228 & 1.350 & 0.375 & 0.604 & 1.318 & 0.810 & 1.884 & 1.259 & 2.589 & 3.477 \\ 
  GFT & -- & -- & -- & 1.106 & 1.196 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.436 & 0.419 & \textbf{0.385} & \textbf{0.241} & \textbf{0.264} & 0.165 & 0.346 & 0.797 & 0.612 & \textbf{0.620} & 0.251 & 0.598 & 0.366 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & 0.243 & \textbf{0.240} & 0.235 & 0.183 & 0.211 & 0.109 & 0.227 & 0.476 & \textbf{0.363} & \textbf{0.423} & \textbf{0.161} & 0.374 & \textbf{0.215} \\ 
  ARGOX & \textbf{0.243} & 0.243 & 0.243 & 0.176 & 0.204 & \textbf{0.106} & \textbf{0.223} & 0.479 & 0.365 & 0.453 & 0.164 & 0.374 & 0.229 \\ 
  VAR1 & 0.541 & 0.888 & 1.533 & 0.802 & 0.946 & 0.303 & 0.439 & 0.731 & 0.583 & 1.497 & 1.171 & 1.990 & 2.725 \\ 
  GFT & -- & -- & -- & 0.889 & 0.972 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.258 & 0.248 & \textbf{0.228} & \textbf{0.156} & \textbf{0.181} & 0.116 & 0.242 & \textbf{0.476} & 0.384 & 0.452 & 0.177 & \textbf{0.373} & 0.274 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C &  0.918 & \textbf{ 0.895} &  0.807 &  0.840 &  0.813 &  0.897 &  0.663 & \textbf{ 0.909} &  0.732 &  0.919 &  0.222 &  0.639 & \textbf{ 0.914} \\ 
  ARGOX & \textbf{ 0.919} &  0.893 &  0.793 &  0.858 &  0.835 & \textbf{ 0.904} &  0.688 &  0.907 &  0.743 &  0.906 &  0.232 &  0.636 &  0.906 \\ 
  VAR1 &  0.660 &  0.454 &  0.530 &  0.888 &  0.870 &  0.636 &  0.669 &  0.793 &  0.473 &  0.600 & \textbf{ 0.497} & -0.197 &  0.839 \\ 
  GFT & -- & -- & -- & \textbf{ 0.909} & \textbf{ 0.897} & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive &  0.907 &  0.894 & \textbf{ 0.823} &  0.894 &  0.879 &  0.883 & \textbf{ 0.692} &  0.886 & \textbf{ 0.743} & \textbf{ 0.928} &  0.192 & \textbf{ 0.661} &  0.844 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in New Hampshire.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.NH}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & \textbf{0.446} & \textbf{0.623} & \textbf{0.859} & \textbf{0.470} & \textbf{0.511} & \textbf{0.485} & 0.620 & \textbf{0.716} & \textbf{0.196} & \textbf{1.575} & 0.266 & \textbf{0.810} & \textbf{0.773} \\ 
  ARGOX & 0.461 & 0.638 & 0.876 & 0.498 & 0.541 & 0.485 & 0.676 & 0.718 & 0.238 & 1.590 & 0.252 & 0.848 & 0.812 \\ 
  VAR1 & 1.548 & 1.842 & 2.290 & 1.157 & 1.221 & 1.580 & 2.953 & 1.932 & 1.062 & 4.069 & 1.344 & 1.738 & 2.497 \\ 
  GFT & -- & -- & -- & 0.828 & 0.860 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.566 & 0.704 & 0.905 & 0.593 & 0.641 & 0.503 & \textbf{0.605} & 1.004 & 0.431 & 1.625 & \textbf{0.234} & 0.973 & 0.947 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & \textbf{0.319} & \textbf{0.352} & \textbf{0.413} & \textbf{0.367} & \textbf{0.410} & 0.381 & 0.510 & 0.526 & \textbf{0.165} & 0.892 & 0.206 & \textbf{0.466} & \textbf{0.590} \\ 
  ARGOX & 0.322 & 0.356 & 0.419 & 0.386 & 0.435 & 0.381 & 0.552 & \textbf{0.506} & 0.195 & \textbf{0.876} & 0.193 & 0.485 & 0.636 \\ 
  VAR1 & 1.145 & 1.248 & 1.439 & 0.987 & 1.035 & 1.231 & 2.780 & 1.316 & 0.941 & 2.654 & 1.268 & 1.166 & 2.084 \\ 
  GFT & -- & -- & -- & 0.688 & 0.699 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.361 & 0.402 & 0.477 & 0.438 & 0.483 & \textbf{0.376} & \textbf{0.456} & 0.609 & 0.303 & 1.113 & \textbf{0.182} & 0.556 & 0.783 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & \textbf{0.972} & \textbf{0.959} & \textbf{0.944} & \textbf{0.895} & \textbf{0.879} & 0.922 & \textbf{0.927} & 0.969 & \textbf{0.988} & \textbf{0.916} & \textbf{0.889} & \textbf{0.895} & \textbf{0.934} \\ 
  ARGOX & 0.970 & 0.957 & 0.942 & 0.884 & 0.866 & \textbf{0.923} & 0.910 & \textbf{0.970} & 0.982 & 0.915 & 0.882 & 0.883 & 0.928 \\ 
  VAR1 & 0.790 & 0.728 & 0.648 & 0.802 & 0.771 & 0.580 & 0.777 & 0.827 & 0.898 & 0.409 & 0.370 & 0.525 & 0.617 \\ 
  GFT & -- & -- & -- & 0.888 & 0.872 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.955 & 0.947 & 0.937 & 0.837 & 0.810 & 0.909 & 0.917 & 0.929 & 0.940 & 0.901 & 0.881 & 0.831 & 0.892 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in New Jersey.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.NJ}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & 0.502 & \textbf{0.573} & \textbf{0.685} & \textbf{0.430} & \textbf{0.466} & \textbf{0.449} & 0.362 & 0.731 & 0.586 & \textbf{0.856} & \textbf{0.248} & 0.535 & \textbf{1.687} \\ 
  ARGOX & \textbf{0.498} & 0.574 & 0.694 & 0.449 & 0.488 & 0.465 & \textbf{0.347} & \textbf{0.689} & \textbf{0.567} & 0.928 & 0.249 & \textbf{0.498} & 1.691 \\ 
  VAR1 & 2.238 & 2.942 & 3.927 & 2.220 & 2.402 & 2.092 & 1.849 & 2.396 & 2.605 & 4.151 & 1.208 & 3.901 & 9.287 \\ 
  GFT & -- & -- & -- & 1.456 & 1.510 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.647 & 0.726 & 0.852 & 0.665 & 0.729 & 0.484 & 0.409 & 0.911 & 0.749 & 1.136 & 0.256 & 0.706 & 2.174 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & 0.329 & 0.355 & \textbf{0.402} & 0.304 & 0.335 & \textbf{0.345} & 0.267 & 0.441 & 0.390 & \textbf{0.637} & \textbf{0.195} & 0.412 & \textbf{1.270} \\ 
  ARGOX & \textbf{0.322} & \textbf{0.351} & 0.405 & \textbf{0.299} & \textbf{0.331} & 0.360 & \textbf{0.244} & \textbf{0.415} & \textbf{0.381} & 0.678 & 0.197 & \textbf{0.393} & 1.271 \\ 
  VAR1 & 1.610 & 2.016 & 2.769 & 1.886 & 2.080 & 1.831 & 1.560 & 1.692 & 2.070 & 3.290 & 1.137 & 3.667 & 7.937 \\ 
  GFT & -- & -- & -- & 1.285 & 1.322 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.389 & 0.418 & 0.471 & 0.392 & 0.443 & 0.368 & 0.310 & 0.592 & 0.501 & 0.759 & 0.201 & 0.533 & 1.618 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & 0.967 & \textbf{0.972} & \textbf{0.975} & \textbf{0.948} & 0.938 & \textbf{0.929} & 0.949 & 0.952 & 0.955 & \textbf{0.962} & \textbf{0.837} & 0.935 & \textbf{0.952} \\ 
  ARGOX & \textbf{0.967} & 0.971 & 0.973 & 0.943 & 0.933 & 0.923 & \textbf{0.953} & \textbf{0.958} & \textbf{0.957} & 0.956 & 0.834 & \textbf{0.946} & 0.947 \\ 
  VAR1 & 0.675 & 0.500 & 0.493 & 0.480 & 0.376 & 0.661 & 0.530 & 0.710 & 0.696 & 0.636 & 0.272 & 0.455 & 0.451 \\ 
  GFT & -- & -- & -- & 0.947 & \textbf{0.943} & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.945 & 0.954 & 0.959 & 0.868 & 0.841 & 0.916 & 0.935 & 0.924 & 0.924 & 0.932 & 0.813 & 0.887 & 0.907 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in New Mexico.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.NM}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & \textbf{0.585} & \textbf{0.575} & 0.555 & \textbf{0.665} & \textbf{0.702} & 0.523 & \textbf{0.990} & 0.801 & 0.321 & 0.871 & 0.179 & 0.444 & \textbf{1.103} \\ 
  ARGOX & 0.589 & 0.576 & \textbf{0.551} & 0.690 & 0.734 & \textbf{0.520} & 1.064 & \textbf{0.719} & \textbf{0.294} & \textbf{0.839} & 0.167 & 0.447 & 1.131 \\ 
  VAR1 & 1.260 & 1.593 & 2.074 & 1.217 & 1.310 & 0.886 & 1.402 & 1.417 & 1.764 & 3.741 & 1.135 & 1.597 & 1.939 \\ 
  GFT & -- & -- & -- & 0.860 & 0.916 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.688 & 0.669 & 0.632 & 0.838 & 0.899 & 0.580 & 1.060 & 0.992 & 0.379 & 1.044 & \textbf{0.150} & \textbf{0.430} & 1.384 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & 0.392 & 0.362 & 0.306 & \textbf{0.502} & \textbf{0.517} & 0.413 & 0.750 & 0.582 & 0.233 & 0.565 & 0.143 & 0.317 & \textbf{0.866} \\ 
  ARGOX & \textbf{0.390} & \textbf{0.360} & \textbf{0.304} & 0.513 & 0.534 & \textbf{0.401} & 0.781 & \textbf{0.546} & \textbf{0.232} & \textbf{0.552} & 0.137 & \textbf{0.315} & 0.902 \\ 
  VAR1 & 1.010 & 1.145 & 1.394 & 0.858 & 0.942 & 0.694 & 1.161 & 1.002 & 1.690 & 2.529 & 1.079 & 1.114 & 1.763 \\ 
  GFT & -- & -- & -- & 0.651 & 0.696 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.415 & 0.391 & 0.347 & 0.553 & 0.588 & 0.432 & \textbf{0.732} & 0.662 & 0.291 & 0.775 & \textbf{0.119} & 0.339 & 1.146 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & \textbf{0.960} & \textbf{0.954} & 0.937 & \textbf{0.926} & \textbf{0.926} & \textbf{0.825} & \textbf{0.928} & 0.963 & 0.956 & 0.936 & 0.758 & \textbf{0.909} & 0.802 \\ 
  ARGOX & 0.959 & 0.954 & \textbf{0.938} & 0.922 & 0.920 & 0.822 & 0.916 & \textbf{0.972} & \textbf{0.962} & \textbf{0.943} & 0.769 & 0.898 & 0.791 \\ 
  VAR1 & 0.841 & 0.784 & 0.830 & 0.870 & 0.870 & 0.618 & 0.926 & 0.880 & 0.905 & 0.684 & 0.705 & 0.681 & \textbf{0.867} \\ 
  GFT & -- & -- & -- & 0.900 & 0.894 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.945 & 0.939 & 0.921 & 0.886 & 0.878 & 0.794 & 0.915 & 0.942 & 0.940 & 0.901 & \textbf{0.814} & 0.867 & 0.702 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in New York.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.NY}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & \textbf{0.460} & \textbf{0.428} & \textbf{0.363} & \textbf{0.537} & \textbf{0.589} & \textbf{0.344} & \textbf{0.711} & \textbf{0.716} & 0.335 & 0.372 & 0.121 & \textbf{0.202} & \textbf{0.941} \\ 
  ARGOX & 0.492 & 0.458 & 0.387 & 0.696 & 0.765 & 0.359 & 0.726 & 0.739 & \textbf{0.328} & \textbf{0.352} & 0.112 & 0.205 & 1.012 \\ 
  VAR1 & 1.197 & 1.910 & 2.785 & 1.171 & 1.250 & 0.474 & 1.204 & 0.990 & 1.307 & 2.437 & 0.686 & 2.770 & 6.903 \\ 
  GFT & -- & -- & -- & 0.644 & 0.704 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.693 & 0.617 & 0.442 & 1.022 & 1.125 & 0.456 & 0.917 & 1.065 & 0.541 & 0.634 & \textbf{0.093} & 0.324 & 1.078 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & \textbf{0.292} & \textbf{0.256} & \textbf{0.189} & \textbf{0.372} & \textbf{0.434} & \textbf{0.268} & \textbf{0.478} & \textbf{0.466} & 0.210 & 0.277 & 0.091 & 0.166 & \textbf{0.635} \\ 
  ARGOX & 0.297 & 0.262 & 0.197 & 0.421 & 0.497 & 0.269 & 0.495 & 0.500 & \textbf{0.190} & \textbf{0.236} & 0.085 & \textbf{0.163} & 0.725 \\ 
  VAR1 & 0.772 & 1.079 & 1.647 & 0.849 & 0.887 & 0.392 & 0.892 & 0.719 & 0.987 & 1.639 & 0.617 & 2.539 & 5.125 \\ 
  GFT & -- & -- & -- & 0.452 & 0.510 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.409 & 0.343 & 0.221 & 0.509 & 0.606 & 0.348 & 0.680 & 0.725 & 0.374 & 0.454 & \textbf{0.079} & 0.204 & 0.781 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & \textbf{0.967} & \textbf{0.966} & \textbf{0.964} & 0.964 & 0.960 & \textbf{0.937} & 0.929 & \textbf{0.962} & \textbf{0.983} & 0.977 & 0.942 & \textbf{0.971} & \textbf{0.870} \\ 
  ARGOX & 0.962 & 0.961 & 0.960 & 0.936 & 0.928 & 0.930 & 0.927 & 0.959 & 0.980 & \textbf{0.979} & \textbf{0.950} & 0.967 & 0.852 \\ 
  VAR1 & 0.795 & 0.670 & 0.690 & 0.823 & 0.796 & 0.897 & \textbf{0.936} & 0.919 & 0.759 & 0.848 & 0.674 & 0.646 & 0.163 \\ 
  GFT & -- & -- & -- & \textbf{0.976} & \textbf{0.972} & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.923 & 0.930 & 0.948 & 0.852 & 0.831 & 0.881 & 0.881 & 0.908 & 0.940 & 0.925 & 0.935 & 0.896 & 0.833 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in North Carolina.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.NC}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & \textbf{0.767} & \textbf{0.889} & \textbf{1.079} & \textbf{0.899} & \textbf{0.990} & \textbf{0.432} & \textbf{1.099} & 0.776 & \textbf{0.610} & \textbf{1.284} & \textbf{0.394} & \textbf{0.999} & \textbf{2.578} \\ 
  ARGOX & 0.786 & 0.911 & 1.106 & 0.902 & 0.992 & 0.435 & 1.114 & 0.796 & 0.648 & 1.335 & 0.396 & 1.061 & 2.631 \\ 
  VAR1 & 1.158 & 1.427 & 1.824 & 1.061 & 1.161 & 0.618 & 1.377 & \textbf{0.729} & 0.885 & 2.886 & 0.855 & 1.935 & 3.853 \\ 
  GFT & -- & -- & -- & 1.020 & 1.112 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.891 & 1.011 & 1.202 & 0.960 & 1.056 & 0.495 & 1.342 & 0.988 & 0.775 & 1.480 & 0.412 & 1.077 & 2.861 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & \textbf{0.478} & \textbf{0.513} & \textbf{0.576} & \textbf{0.510} & \textbf{0.606} & \textbf{0.353} & \textbf{0.761} & 0.596 & \textbf{0.459} & \textbf{0.915} & \textbf{0.301} & \textbf{0.645} & \textbf{1.610} \\ 
  ARGOX & 0.491 & 0.526 & 0.591 & 0.512 & 0.608 & 0.357 & 0.776 & 0.622 & 0.489 & 0.966 & 0.301 & 0.686 & 1.644 \\ 
  VAR1 & 0.696 & 0.815 & 1.035 & 0.632 & 0.709 & 0.479 & 1.033 & \textbf{0.585} & 0.605 & 2.112 & 0.641 & 1.161 & 2.691 \\ 
  GFT & -- & -- & -- & 0.709 & 0.788 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.556 & 0.603 & 0.690 & 0.557 & 0.663 & 0.405 & 0.899 & 0.720 & 0.604 & 1.128 & 0.340 & 0.799 & 1.949 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & \textbf{ 0.875} & \textbf{ 0.868} & \textbf{ 0.847} &  0.870 &  0.850 & \textbf{ 0.739} & \textbf{ 0.670} &  0.867 & \textbf{ 0.881} & \textbf{ 0.835} &  0.744 & \textbf{ 0.877} &  0.700 \\ 
  ARGOX &  0.869 &  0.862 &  0.840 &  0.869 &  0.849 &  0.733 &  0.661 &  0.857 &  0.862 &  0.822 &  0.746 &  0.857 &  0.695 \\ 
  VAR1 &  0.726 &  0.672 &  0.570 & \textbf{ 0.887} & \textbf{ 0.871} &  0.580 &  0.567 & \textbf{ 0.901} &  0.753 &  0.331 & -0.046 &  0.704 & \textbf{ 0.804} \\ 
  GFT & -- & -- & -- &  0.834 &  0.808 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive &  0.839 &  0.840 &  0.826 &  0.859 &  0.839 &  0.687 &  0.575 &  0.748 &  0.814 &  0.793 & \textbf{ 0.768} &  0.859 &  0.675 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in North Dakota.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.ND}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & \textbf{0.301} & \textbf{0.343} & \textbf{0.410} & \textbf{0.517} & \textbf{0.568} & 0.222 & \textbf{0.235} & \textbf{0.347} & 0.317 & \textbf{0.416} & 0.187 & \textbf{0.407} & \textbf{0.888} \\ 
  ARGOX & 0.321 & 0.374 & 0.455 & 0.580 & 0.636 & \textbf{0.214} & 0.239 & 0.352 & \textbf{0.315} & 0.478 & \textbf{0.187} & 0.436 & 1.015 \\ 
  VAR1 & 1.528 & 1.458 & 1.320 & 1.907 & 2.055 & 0.733 & 2.348 & 2.549 & 0.952 & 2.274 & 0.248 & 0.911 & 2.513 \\ 
  GFT & -- & -- & -- & 0.954 & 1.039 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.426 & 0.473 & 0.549 & 0.783 & 0.861 & 0.255 & 0.322 & 0.526 & 0.379 & 0.515 & 0.189 & 0.515 & 1.334 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & \textbf{0.185} & \textbf{0.210} & \textbf{0.256} & \textbf{0.243} & \textbf{0.278} & 0.159 & \textbf{0.175} & 0.251 & 0.236 & \textbf{0.307} & \textbf{0.138} & \textbf{0.335} & \textbf{0.631} \\ 
  ARGOX & 0.190 & 0.219 & 0.273 & 0.284 & 0.320 & \textbf{0.148} & 0.178 & \textbf{0.244} & \textbf{0.227} & 0.316 & 0.141 & 0.351 & 0.742 \\ 
  VAR1 & 0.994 & 0.892 & 0.702 & 1.424 & 1.548 & 0.570 & 1.763 & 1.807 & 0.758 & 1.571 & 0.200 & 0.752 & 1.910 \\ 
  GFT & -- & -- & -- & 0.774 & 0.870 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.233 & 0.261 & 0.314 & 0.388 & 0.453 & 0.192 & 0.225 & 0.339 & 0.268 & 0.391 & 0.142 & 0.408 & 0.951 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & \textbf{0.951} & \textbf{0.972} & \textbf{0.976} & 0.925 & 0.920 & 0.866 & \textbf{0.961} & \textbf{0.962} & 0.899 & \textbf{0.939} & 0.750 & \textbf{0.930} & \textbf{0.952} \\ 
  ARGOX & 0.944 & 0.966 & 0.970 & 0.903 & 0.896 & \textbf{0.880} & 0.959 & 0.961 & \textbf{0.899} & 0.918 & \textbf{0.751} & 0.916 & 0.934 \\ 
  VAR1 & 0.777 & 0.648 & 0.721 & 0.431 & 0.376 & 0.838 & 0.882 & 0.867 & 0.789 & 0.656 & 0.573 & 0.810 & 0.727 \\ 
  GFT & -- & -- & -- & \textbf{0.971} & \textbf{0.969} & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.903 & 0.946 & 0.957 & 0.826 & 0.811 & 0.835 & 0.922 & 0.910 & 0.860 & 0.899 & 0.744 & 0.878 & 0.887 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in Ohio.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.OH}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & 0.955 & 0.901 & \textbf{0.790} & 1.444 & 1.576 & 0.890 & 1.552 & 0.853 & \textbf{0.725} & \textbf{1.018} & 0.579 & 1.014 & \textbf{1.099} \\ 
  ARGOX & \textbf{0.933} & \textbf{0.889} & 0.801 & 1.435 & 1.564 & 0.887 & 1.500 & \textbf{0.733} & 0.747 & 1.068 & \textbf{0.577} & \textbf{0.996} & 1.121 \\ 
  VAR1 & 3.239 & 2.751 & 1.465 & 4.118 & 4.533 & 2.011 & 5.221 & 3.008 & 3.988 & 4.228 & 0.960 & 1.142 & 1.758 \\ 
  GFT & -- & -- & -- & 2.056 & 2.208 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.987 & 0.925 & 0.796 & \textbf{1.375} & \textbf{1.508} & \textbf{0.887} & \textbf{1.457} & 1.015 & 0.994 & 1.176 & 0.618 & 1.002 & 1.130 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & 0.601 & 0.573 & \textbf{0.523} & 0.982 & \textbf{1.119} & 0.726 & 1.087 & 0.598 & \textbf{0.495} & \textbf{0.685} & \textbf{0.451} & 0.656 & \textbf{0.761} \\ 
  ARGOX & \textbf{0.589} & \textbf{0.569} & 0.532 & 0.996 & 1.126 & 0.724 & \textbf{1.050} & \textbf{0.536} & 0.508 & 0.707 & 0.456 & \textbf{0.640} & 0.816 \\ 
  VAR1 & 2.027 & 1.678 & 1.032 & 2.770 & 3.328 & 1.801 & 3.975 & 2.103 & 3.007 & 3.647 & 0.784 & 0.973 & 1.506 \\ 
  GFT & -- & -- & -- & 1.424 & 1.504 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.650 & 0.609 & 0.533 & \textbf{0.970} & 1.123 & \textbf{0.716} & 1.091 & 0.763 & 0.706 & 0.812 & 0.500 & 0.692 & 0.916 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & 0.952 & 0.947 & 0.915 & 0.914 & 0.892 & 0.506 & 0.921 & 0.972 & \textbf{0.973} & \textbf{0.941} & 0.774 & 0.533 & \textbf{0.915} \\ 
  ARGOX & \textbf{0.955} & \textbf{0.949} & 0.913 & 0.917 & 0.897 & 0.498 & 0.925 & \textbf{0.978} & 0.971 & 0.935 & \textbf{0.777} & 0.529 & 0.909 \\ 
  VAR1 & 0.709 & 0.491 & 0.709 & 0.541 & 0.479 & 0.257 & 0.743 & 0.765 & 0.513 & 0.864 & 0.571 & 0.431 & 0.869 \\ 
  GFT & -- & -- & -- & 0.842 & 0.809 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.950 & 0.946 & \textbf{0.919} & \textbf{0.923} & \textbf{0.904} & \textbf{0.535} & \textbf{0.931} & 0.941 & 0.940 & 0.921 & 0.751 & \textbf{0.534} & 0.898 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in Oklahoma.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.OK}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & 0.428 & 0.397 & 0.332 & 0.371 & 0.402 & \textbf{0.569} & 0.817 & 0.339 & \textbf{0.358} & 0.413 & 0.158 & 0.222 & \textbf{0.775} \\ 
  ARGOX & \textbf{0.425} & \textbf{0.393} & \textbf{0.324} & 0.368 & 0.399 & 0.579 & \textbf{0.810} & \textbf{0.290} & 0.367 & \textbf{0.387} & 0.144 & \textbf{0.197} & 0.804 \\ 
  VAR1 & 2.425 & 2.061 & 1.102 & 3.854 & 4.239 & 1.258 & 3.884 & 2.004 & 2.512 & 2.624 & 0.986 & 1.147 & 1.567 \\ 
  GFT & -- & -- & -- & 0.570 & 0.487 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.500 & 0.478 & 0.433 & \textbf{0.323} & \textbf{0.348} & 0.632 & 0.946 & 0.442 & 0.450 & 0.757 & \textbf{0.127} & 0.283 & 0.891 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & 0.260 & 0.237 & 0.195 & 0.275 & 0.306 & \textbf{0.419} & 0.465 & 0.231 & \textbf{0.253} & \textbf{0.296} & 0.120 & 0.177 & \textbf{0.580} \\ 
  ARGOX & \textbf{0.258} & \textbf{0.234} & \textbf{0.188} & 0.273 & 0.303 & 0.429 & \textbf{0.464} & \textbf{0.205} & 0.265 & 0.297 & 0.114 & \textbf{0.161} & 0.589 \\ 
  VAR1 & 1.527 & 1.253 & 0.745 & 2.792 & 3.300 & 1.129 & 2.993 & 1.324 & 2.038 & 2.044 & 0.781 & 0.927 & 1.275 \\ 
  GFT & -- & -- & -- & 0.473 & 0.396 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.292 & 0.273 & 0.238 & \textbf{0.254} & \textbf{0.280} & 0.428 & 0.560 & 0.319 & 0.275 & 0.580 & \textbf{0.097} & 0.189 & 0.672 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & 0.940 & 0.945 & 0.959 & 0.794 & 0.726 & \textbf{0.741} & 0.781 & 0.983 & \textbf{0.953} & 0.969 & 0.938 & 0.919 & \textbf{0.900} \\ 
  ARGOX & \textbf{0.940} & \textbf{0.946} & \textbf{0.960} & 0.795 & 0.724 & 0.731 & \textbf{0.781} & \textbf{0.986} & 0.952 & \textbf{0.973} & \textbf{0.945} & \textbf{0.936} & 0.889 \\ 
  VAR1 & 0.727 & 0.720 & 0.823 & 0.593 & 0.469 & 0.658 & 0.579 & 0.917 & 0.856 & 0.713 & 0.533 & 0.405 & 0.763 \\ 
  GFT & -- & -- & -- & 0.755 & \textbf{0.822} & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.918 & 0.922 & 0.931 & \textbf{0.799} & 0.737 & 0.713 & 0.728 & 0.950 & 0.919 & 0.892 & 0.939 & 0.874 & 0.867 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in Oregon.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.OR}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & \textbf{0.328} & \textbf{0.306} & 0.262 & \textbf{0.492} & \textbf{0.529} & 0.341 & \textbf{0.431} & 0.413 & 0.190 & 0.442 & 0.143 & \textbf{0.261} & \textbf{0.322} \\ 
  ARGOX & 0.336 & 0.309 & \textbf{0.250} & 0.535 & 0.575 & \textbf{0.332} & 0.456 & \textbf{0.388} & \textbf{0.190} & \textbf{0.404} & \textbf{0.131} & 0.264 & 0.352 \\ 
  VAR1 & 1.117 & 0.962 & 0.574 & 2.077 & 2.247 & 1.147 & 1.112 & 1.065 & 0.706 & 0.878 & 0.209 & 0.670 & 1.090 \\ 
  GFT & -- & -- & -- & 0.589 & 0.640 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.465 & 0.429 & 0.354 & 0.764 & 0.832 & 0.454 & 0.564 & 0.573 & 0.286 & 0.673 & 0.138 & 0.340 & 0.498 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & \textbf{0.216} & 0.193 & 0.151 & \textbf{0.340} & \textbf{0.365} & 0.250 & \textbf{0.314} & 0.267 & \textbf{0.146} & 0.241 & 0.105 & 0.183 & \textbf{0.241} \\ 
  ARGOX & 0.216 & \textbf{0.191} & \textbf{0.145} & 0.366 & 0.393 & \textbf{0.241} & 0.329 & \textbf{0.235} & 0.153 & \textbf{0.235} & \textbf{0.097} & \textbf{0.169} & 0.259 \\ 
  VAR1 & 0.751 & 0.626 & 0.392 & 1.605 & 1.757 & 1.019 & 0.859 & 0.587 & 0.546 & 0.660 & 0.168 & 0.491 & 0.981 \\ 
  GFT & -- & -- & -- & 0.480 & 0.535 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.288 & 0.256 & 0.197 & 0.504 & 0.565 & 0.336 & 0.396 & 0.368 & 0.212 & 0.500 & 0.101 & 0.211 & 0.376 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & \textbf{0.969} & \textbf{0.969} & 0.967 & \textbf{0.951} & \textbf{0.949} & 0.871 & \textbf{0.940} & 0.977 & 0.977 & 0.961 & 0.917 & \textbf{0.965} & \textbf{0.958} \\ 
  ARGOX & 0.968 & 0.969 & \textbf{0.971} & 0.943 & 0.940 & \textbf{0.877} & 0.932 & \textbf{0.982} & \textbf{0.978} & \textbf{0.969} & \textbf{0.926} & 0.956 & 0.948 \\ 
  VAR1 & 0.707 & 0.719 & 0.871 & 0.714 & 0.678 & 0.669 & 0.705 & 0.808 & 0.746 & 0.845 & 0.824 & 0.412 & 0.805 \\ 
  GFT & -- & -- & -- & 0.946 & 0.942 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.937 & 0.940 & 0.943 & 0.880 & 0.867 & 0.793 & 0.900 & 0.944 & 0.943 & 0.904 & 0.915 & 0.869 & 0.892 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in Pennsylvania.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.PA}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & \textbf{0.445} & \textbf{0.473} & 0.522 & \textbf{0.475} & \textbf{0.522} & \textbf{0.225} & \textbf{0.471} & 0.639 & \textbf{0.509} & \textbf{0.911} & 0.149 & 0.595 & 0.899 \\ 
  ARGOX & 0.457 & 0.488 & 0.539 & 0.483 & 0.531 & 0.232 & 0.486 & \textbf{0.638} & 0.520 & 1.003 & 0.144 & 0.579 & \textbf{0.897} \\ 
  VAR1 & 1.227 & 1.181 & 1.090 & 1.614 & 1.707 & 1.538 & 0.914 & 0.907 & 1.226 & 2.481 & 0.523 & 0.790 & 1.319 \\ 
  GFT & -- & -- & -- & 0.674 & 0.709 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.542 & 0.528 & \textbf{0.501} & 0.475 & 0.522 & 0.239 & 0.542 & 0.825 & 0.654 & 0.959 & \textbf{0.135} & \textbf{0.577} & 1.051 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & \textbf{0.260} & \textbf{0.265} & 0.276 & \textbf{0.261} & \textbf{0.305} & 0.164 & \textbf{0.315} & 0.468 & \textbf{0.362} & \textbf{0.556} & 0.121 & 0.409 & \textbf{0.595} \\ 
  ARGOX & 0.266 & 0.270 & 0.279 & 0.270 & 0.313 & 0.169 & 0.325 & \textbf{0.465} & 0.372 & 0.607 & 0.118 & 0.396 & 0.625 \\ 
  VAR1 & 0.976 & 0.877 & 0.693 & 1.376 & 1.445 & 1.480 & 0.785 & 0.696 & 0.913 & 1.910 & 0.466 & 0.596 & 1.021 \\ 
  GFT & -- & -- & -- & 0.593 & 0.619 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.304 & 0.289 & \textbf{0.261} & 0.285 & 0.335 & \textbf{0.153} & 0.365 & 0.578 & 0.490 & 0.618 & \textbf{0.105} & \textbf{0.376} & 0.725 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & \textbf{0.969} & \textbf{0.954} & 0.906 & 0.916 & 0.906 & \textbf{0.920} & \textbf{0.935} & 0.952 & \textbf{0.963} & \textbf{0.950} & 0.776 & \textbf{0.626} & 0.928 \\ 
  ARGOX & 0.967 & 0.951 & 0.900 & 0.914 & 0.905 & 0.913 & 0.928 & \textbf{0.953} & 0.960 & 0.940 & \textbf{0.802} & 0.626 & 0.928 \\ 
  VAR1 & 0.787 & 0.746 & 0.630 & 0.763 & 0.735 & 0.767 & 0.890 & 0.900 & 0.867 & 0.549 & 0.702 & 0.333 & \textbf{0.933} \\ 
  GFT & -- & -- & -- & \textbf{0.943} & \textbf{0.937} & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.951 & 0.944 & \textbf{0.919} & 0.911 & 0.901 & 0.907 & 0.904 & 0.915 & 0.936 & 0.946 & 0.746 & 0.589 & 0.890 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in Rhode Island.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.RI}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & \textbf{0.567} & \textbf{0.583} & \textbf{0.612} & \textbf{0.512} & \textbf{0.560} & 0.332 & \textbf{0.913} & \textbf{0.679} & 0.689 & \textbf{0.790} & 0.338 & \textbf{0.316} & \textbf{1.498} \\ 
  ARGOX & 0.594 & 0.620 & 0.665 & 0.593 & 0.648 & \textbf{0.330} & 0.942 & 0.709 & \textbf{0.682} & 0.858 & 0.320 & 0.319 & 1.683 \\ 
  VAR1 & 2.333 & 2.324 & 2.308 & 1.559 & 1.715 & 0.799 & 2.941 & 4.113 & 2.165 & 4.152 & 1.123 & 1.449 & 5.240 \\ 
  GFT & -- & -- & -- & 1.584 & 1.725 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.875 & 0.841 & 0.775 & 0.796 & 0.873 & 0.376 & 1.006 & 1.358 & 0.933 & 1.589 & \textbf{0.246} & 0.503 & 1.788 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & \textbf{0.347} & \textbf{0.352} & \textbf{0.362} & \textbf{0.265} & \textbf{0.301} & \textbf{0.258} & \textbf{0.733} & \textbf{0.447} & \textbf{0.433} & \textbf{0.578} & 0.270 & 0.238 & \textbf{1.081} \\ 
  ARGOX & 0.363 & 0.364 & 0.366 & 0.284 & 0.317 & 0.261 & 0.763 & 0.457 & 0.450 & 0.622 & 0.243 & \textbf{0.222} & 1.258 \\ 
  VAR1 & 1.471 & 1.486 & 1.513 & 0.834 & 0.989 & 0.633 & 2.505 & 3.045 & 1.807 & 3.584 & 0.987 & 1.136 & 3.904 \\ 
  GFT & -- & -- & -- & 1.319 & 1.483 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.514 & 0.481 & 0.420 & 0.421 & 0.481 & 0.292 & 0.795 & 0.903 & 0.683 & 1.174 & \textbf{0.195} & 0.342 & 1.365 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & \textbf{ 0.980} & \textbf{ 0.975} & \textbf{ 0.961} &  0.944 &  0.939 &  0.855 & \textbf{ 0.913} & \textbf{ 0.985} & \textbf{ 0.961} & \textbf{ 0.970} &  0.920 & \textbf{ 0.979} & \textbf{ 0.849} \\ 
  ARGOX &  0.978 &  0.972 &  0.955 &  0.919 &  0.910 & \textbf{ 0.856} &  0.906 &  0.984 &  0.958 &  0.965 & \textbf{ 0.931} &  0.971 &  0.813 \\ 
  VAR1 &  0.782 &  0.737 &  0.596 &  0.295 &  0.208 &  0.600 &  0.711 &  0.751 &  0.840 &  0.753 &  0.758 &  0.563 & -0.169 \\ 
  GFT & -- & -- & -- & \textbf{ 0.977} & \textbf{ 0.975} & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive &  0.952 &  0.949 &  0.939 &  0.851 &  0.834 &  0.823 &  0.888 &  0.939 &  0.915 &  0.878 &  0.930 &  0.905 &  0.791 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in South Carolina.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.SC}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & \textbf{0.326} & \textbf{0.306} & \textbf{0.265} & \textbf{0.315} & \textbf{0.329} & \textbf{0.292} & \textbf{0.418} & \textbf{0.492} & \textbf{0.358} & \textbf{0.355} & 0.182 & \textbf{0.283} & \textbf{0.430} \\ 
  ARGOX & 0.329 & 0.310 & 0.270 & 0.318 & 0.332 & 0.295 & 0.425 & 0.495 & 0.362 & 0.368 & \textbf{0.179} & 0.288 & 0.443 \\ 
  VAR1 & 2.064 & 2.162 & 2.333 & 0.832 & 0.888 & 0.722 & 1.882 & 3.319 & 2.914 & 4.225 & 1.169 & 1.176 & 5.356 \\ 
  GFT & -- & -- & -- & 1.033 & 1.132 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.354 & 0.330 & 0.282 & 0.362 & 0.380 & 0.309 & 0.427 & 0.542 & 0.376 & 0.403 & 0.184 & 0.302 & 0.468 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & \textbf{0.233} & \textbf{0.215} & \textbf{0.183} & \textbf{0.235} & \textbf{0.243} & 0.218 & \textbf{0.297} & \textbf{0.369} & \textbf{0.279} & \textbf{0.233} & 0.148 & \textbf{0.204} & \textbf{0.336} \\ 
  ARGOX & 0.235 & 0.217 & 0.184 & 0.238 & 0.245 & \textbf{0.217} & 0.299 & 0.371 & 0.283 & 0.247 & \textbf{0.147} & 0.209 & 0.350 \\ 
  VAR1 & 1.264 & 1.352 & 1.514 & 0.588 & 0.615 & 0.559 & 1.481 & 2.117 & 2.444 & 3.700 & 0.978 & 0.965 & 4.631 \\ 
  GFT & -- & -- & -- & 0.512 & 0.584 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.257 & 0.233 & 0.188 & 0.263 & 0.270 & 0.244 & 0.318 & 0.428 & 0.284 & 0.257 & 0.154 & 0.226 & 0.367 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & \textbf{ 0.950} & \textbf{ 0.950} & \textbf{ 0.937} & \textbf{ 0.921} & \textbf{ 0.912} & \textbf{ 0.851} & \textbf{ 0.925} & \textbf{ 0.923} & \textbf{ 0.876} & \textbf{ 0.960} & \textbf{ 0.381} & \textbf{ 0.907} & \textbf{ 0.905} \\ 
  ARGOX &  0.949 &  0.949 &  0.933 &  0.919 &  0.910 &  0.847 &  0.923 &  0.922 &  0.873 &  0.957 &  0.380 &  0.902 &  0.898 \\ 
  VAR1 &  0.812 &  0.750 &  0.702 &  0.806 &  0.780 &  0.434 &  0.759 &  0.906 &  0.851 &  0.849 & -0.145 &  0.803 &  0.359 \\ 
  GFT & -- & -- & -- &  0.898 &  0.886 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive &  0.941 &  0.941 &  0.925 &  0.898 &  0.885 &  0.840 &  0.924 &  0.903 &  0.844 &  0.948 &  0.378 &  0.893 &  0.880 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in South Dakota.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.SD}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & \textbf{0.703} & \textbf{0.683} & \textbf{0.644} & \textbf{0.572} & \textbf{0.620} & \textbf{0.478} & 0.883 & 1.061 & \textbf{0.467} & \textbf{1.195} & 0.232 & 0.400 & \textbf{1.620} \\ 
  ARGOX & 0.728 & 0.718 & 0.698 & 0.591 & 0.641 & 0.482 & \textbf{0.870} & \textbf{1.026} & 0.505 & 1.369 & 0.222 & \textbf{0.368} & 1.775 \\ 
  VAR1 & 1.943 & 2.166 & 2.529 & 1.593 & 1.736 & 0.667 & 1.983 & 1.858 & 1.331 & 4.675 & 0.810 & 1.494 & 6.530 \\ 
  GFT & -- & -- & -- & 1.239 & 1.341 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.866 & 0.820 & 0.727 & 0.890 & 0.974 & 0.507 & 0.991 & 1.212 & 0.707 & 1.546 & \textbf{0.126} & 0.512 & 1.837 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & \textbf{0.472} & \textbf{0.429} & \textbf{0.350} & 0.410 & 0.453 & 0.391 & 0.684 & 0.670 & \textbf{0.360} & \textbf{0.896} & 0.176 & 0.249 & \textbf{1.273} \\ 
  ARGOX & 0.477 & 0.438 & 0.365 & \textbf{0.407} & \textbf{0.451} & 0.394 & \textbf{0.663} & \textbf{0.651} & 0.366 & 0.981 & 0.171 & \textbf{0.249} & 1.429 \\ 
  VAR1 & 1.145 & 1.311 & 1.618 & 0.970 & 1.078 & 0.528 & 1.746 & 1.462 & 0.940 & 3.731 & 0.743 & 1.289 & 5.572 \\ 
  GFT & -- & -- & -- & 0.990 & 1.089 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.507 & 0.464 & 0.385 & 0.534 & 0.612 & \textbf{0.358} & 0.711 & 0.726 & 0.522 & 1.055 & \textbf{0.103} & 0.362 & 1.494 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & \textbf{0.951} & \textbf{0.954} & \textbf{0.961} & 0.954 & 0.950 & 0.844 & 0.857 & 0.907 & \textbf{0.950} & \textbf{0.944} & 0.914 & \textbf{0.972} & \textbf{0.891} \\ 
  ARGOX & 0.947 & 0.950 & 0.955 & 0.952 & 0.948 & \textbf{0.844} & 0.862 & \textbf{0.915} & 0.936 & 0.926 & 0.918 & 0.968 & 0.870 \\ 
  VAR1 & 0.658 & 0.604 & 0.672 & 0.695 & 0.656 & 0.770 & \textbf{0.887} & 0.631 & 0.732 & 0.725 & 0.350 & 0.823 & 0.225 \\ 
  GFT & -- & -- & -- & \textbf{0.966} & \textbf{0.964} & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.927 & 0.936 & 0.951 & 0.891 & 0.879 & 0.836 & 0.822 & 0.866 & 0.869 & 0.898 & \textbf{0.932} & 0.902 & 0.861 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in Tennessee.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.TN}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & \textbf{0.851} & \textbf{0.751} & \textbf{0.520} & 1.473 & 1.609 & 0.564 & \textbf{0.761} & 1.087 & 0.647 & \textbf{1.147} & 0.342 & 0.386 & \textbf{0.816} \\ 
  ARGOX & 0.852 & 0.763 & 0.565 & 1.466 & 1.603 & \textbf{0.552} & 0.792 & \textbf{1.049} & \textbf{0.623} & 1.301 & 0.347 & \textbf{0.360} & 0.840 \\ 
  VAR1 & 2.766 & 2.323 & 1.106 & 3.051 & 3.298 & 2.776 & 1.873 & 4.760 & 3.334 & 2.524 & 0.391 & 0.889 & 2.359 \\ 
  GFT & -- & -- & -- & \textbf{1.253} & \textbf{1.368} & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.996 & 0.871 & 0.570 & 1.544 & 1.690 & 0.577 & 0.796 & 1.398 & 0.822 & 1.536 & \textbf{0.338} & 0.555 & 0.841 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & 0.509 & \textbf{0.447} & \textbf{0.331} & 0.848 & 0.953 & 0.451 & \textbf{0.574} & \textbf{0.664} & 0.443 & \textbf{0.833} & 0.264 & \textbf{0.270} & \textbf{0.660} \\ 
  ARGOX & \textbf{0.509} & 0.448 & 0.336 & 0.870 & 0.989 & \textbf{0.448} & 0.590 & 0.671 & \textbf{0.415} & 0.868 & 0.256 & 0.271 & 0.715 \\ 
  VAR1 & 2.134 & 1.637 & 0.717 & 2.567 & 2.819 & 2.411 & 1.319 & 3.934 & 2.974 & 2.063 & 0.276 & 0.736 & 1.752 \\ 
  GFT & -- & -- & -- & \textbf{0.835} & \textbf{0.951} & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.595 & 0.513 & 0.359 & 0.893 & 1.016 & 0.454 & 0.577 & 0.957 & 0.634 & 1.100 & \textbf{0.218} & 0.378 & 0.690 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & \textbf{ 0.961} & \textbf{ 0.963} & \textbf{ 0.967} &  0.860 &  0.837 &  0.824 & \textbf{ 0.953} &  0.970 &  0.973 & \textbf{ 0.955} &  0.568 &  0.928 & \textbf{ 0.923} \\ 
  ARGOX &  0.961 &  0.962 &  0.962 &  0.861 &  0.837 & \textbf{ 0.830} &  0.949 & \textbf{ 0.972} & \textbf{ 0.975} &  0.942 & \textbf{ 0.571} & \textbf{ 0.937} &  0.918 \\ 
  VAR1 &  0.820 &  0.763 &  0.902 &  0.848 &  0.831 & -0.195 &  0.799 &  0.886 &  0.893 &  0.836 &  0.528 &  0.887 &  0.876 \\ 
  GFT & -- & -- & -- & \textbf{ 0.928} & \textbf{ 0.916} & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive &  0.947 &  0.951 &  0.958 &  0.854 &  0.832 &  0.816 &  0.945 &  0.949 &  0.946 &  0.914 &  0.513 &  0.854 &  0.909 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in Texas.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.TX}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & \textbf{0.430} & \textbf{0.410} & \textbf{0.372} & \textbf{0.296} & \textbf{0.312} & \textbf{0.330} & \textbf{0.413} & 0.397 & \textbf{0.619} & \textbf{0.803} & 0.181 & 0.355 & \textbf{0.398} \\ 
  ARGOX & 0.445 & 0.425 & 0.386 & 0.300 & 0.317 & 0.375 & 0.449 & \textbf{0.392} & 0.627 & 0.857 & 0.170 & \textbf{0.338} & 0.458 \\ 
  VAR1 & 3.032 & 2.584 & 1.417 & 2.404 & 2.607 & 1.991 & 3.754 & 6.236 & 1.856 & 3.097 & 0.660 & 0.830 & 3.268 \\ 
  GFT & -- & -- & -- & 1.083 & 1.163 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.507 & 0.489 & 0.454 & 0.512 & 0.550 & 0.429 & 0.439 & 0.451 & 0.658 & 0.997 & \textbf{0.154} & 0.371 & 0.695 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & \textbf{0.296} & \textbf{0.280} & 0.251 & \textbf{0.228} & \textbf{0.240} & \textbf{0.263} & 0.293 & 0.301 & \textbf{0.474} & \textbf{0.583} & 0.148 & 0.277 & \textbf{0.315} \\ 
  ARGOX & 0.302 & 0.282 & \textbf{0.246} & 0.233 & 0.244 & 0.289 & 0.307 & \textbf{0.296} & 0.477 & 0.593 & 0.135 & \textbf{0.260} & 0.348 \\ 
  VAR1 & 2.105 & 1.703 & 0.957 & 1.795 & 1.977 & 1.850 & 2.877 & 5.066 & 1.532 & 2.543 & 0.583 & 0.503 & 2.991 \\ 
  GFT & -- & -- & -- & 1.002 & 1.106 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.334 & 0.313 & 0.273 & 0.355 & 0.381 & 0.329 & \textbf{0.289} & 0.304 & 0.515 & 0.724 & \textbf{0.124} & 0.291 & 0.517 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & \textbf{0.962} & \textbf{0.960} & \textbf{0.957} & \textbf{0.970} & \textbf{0.965} & \textbf{0.930} & \textbf{0.909} & 0.891 & \textbf{0.938} & \textbf{0.938} & 0.601 & \textbf{0.884} & \textbf{0.971} \\ 
  ARGOX & 0.959 & 0.957 & 0.955 & 0.970 & 0.965 & 0.909 & 0.889 & \textbf{0.893} & 0.935 & 0.930 & \textbf{0.617} & 0.876 & 0.957 \\ 
  VAR1 & 0.693 & 0.702 & 0.842 & 0.920 & 0.914 & 0.651 & 0.048 & 0.853 & 0.934 & 0.906 & 0.335 & 0.531 & 0.734 \\ 
  GFT & -- & -- & -- & 0.951 & 0.957 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.947 & 0.945 & 0.937 & 0.911 & 0.894 & 0.885 & 0.889 & 0.868 & 0.921 & 0.899 & 0.541 & 0.809 & 0.894 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in Utah.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.UT}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & 0.493 & \textbf{0.514} & 0.550 & \textbf{0.753} & 0.810 & 0.430 & 0.325 & 0.537 & 0.540 & \textbf{0.545} & \textbf{0.230} & 0.246 & 1.456 \\ 
  ARGOX & \textbf{0.493} & 0.515 & 0.554 & 0.754 & \textbf{0.809} & \textbf{0.429} & \textbf{0.320} & \textbf{0.533} & \textbf{0.539} & 0.555 & 0.232 & 0.248 & 1.468 \\ 
  VAR1 & 1.101 & 1.103 & 1.106 & 1.289 & 1.355 & 0.591 & 0.959 & 1.417 & 1.214 & 1.463 & 0.335 & 1.746 & 1.350 \\ 
  GFT & -- & -- & -- & 1.220 & 1.330 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.536 & 0.531 & \textbf{0.520} & 0.820 & 0.896 & 0.469 & 0.357 & 0.579 & 0.590 & 0.619 & 0.246 & \textbf{0.224} & \textbf{1.325} \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & \textbf{0.348} & \textbf{0.320} & 0.269 & \textbf{0.517} & 0.557 & \textbf{0.324} & 0.257 & \textbf{0.405} & \textbf{0.406} & \textbf{0.387} & \textbf{0.174} & 0.170 & 0.910 \\ 
  ARGOX & 0.348 & 0.320 & \textbf{0.268} & 0.518 & \textbf{0.553} & 0.324 & \textbf{0.254} & 0.406 & 0.409 & 0.389 & 0.175 & 0.168 & 0.915 \\ 
  VAR1 & 0.854 & 0.867 & 0.891 & 0.908 & 0.907 & 0.488 & 0.781 & 1.166 & 1.008 & 1.167 & 0.292 & 1.685 & 1.210 \\ 
  GFT & -- & -- & -- & 0.833 & 0.938 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.381 & 0.342 & 0.271 & 0.560 & 0.639 & 0.360 & 0.264 & 0.450 & 0.447 & 0.445 & 0.187 & \textbf{0.165} & \textbf{0.845} \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & \textbf{0.914} & \textbf{0.902} & 0.863 & 0.904 & 0.872 & 0.790 & 0.797 & 0.920 & 0.878 & \textbf{0.934} & \textbf{0.716} & \textbf{0.773} & 0.691 \\ 
  ARGOX & 0.914 & 0.901 & 0.863 & \textbf{0.904} & \textbf{0.872} & 0.788 & \textbf{0.798} & \textbf{0.921} & \textbf{0.878} & 0.932 & 0.712 & 0.763 & 0.691 \\ 
  VAR1 & 0.618 & 0.616 & 0.730 & 0.763 & 0.693 & \textbf{0.811} & 0.075 & 0.834 & 0.745 & 0.867 & 0.594 & 0.560 & \textbf{0.801} \\ 
  GFT & -- & -- & -- & 0.836 & 0.814 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.901 & 0.897 & \textbf{0.873} & 0.884 & 0.849 & 0.753 & 0.754 & 0.910 & 0.859 & 0.918 & 0.691 & 0.743 & 0.717 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in Vermont.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.VT}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & \textbf{0.418} & \textbf{0.439} & \textbf{0.475} & \textbf{0.623} & \textbf{0.684} & 0.251 & \textbf{0.476} & 0.658 & 0.431 & \textbf{0.364} & 0.149 & \textbf{0.483} & \textbf{0.885} \\ 
  ARGOX & 0.431 & 0.467 & 0.528 & 0.682 & 0.748 & \textbf{0.233} & 0.495 & \textbf{0.636} & \textbf{0.418} & 0.469 & 0.136 & 0.596 & 0.984 \\ 
  VAR1 & 0.638 & 0.761 & 0.947 & 0.933 & 1.026 & 0.289 & 0.688 & 1.023 & 0.565 & 0.926 & \textbf{0.118} & 0.938 & 2.222 \\ 
  GFT & -- & -- & -- & 1.045 & 1.147 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.628 & 0.636 & 0.650 & 0.947 & 1.042 & 0.290 & 0.646 & 0.990 & 0.561 & 0.914 & 0.120 & 0.849 & 1.050 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & \textbf{0.238} & \textbf{0.240} & \textbf{0.243} & \textbf{0.300} & \textbf{0.349} & 0.189 & \textbf{0.319} & 0.443 & 0.292 & \textbf{0.266} & 0.124 & \textbf{0.269} & \textbf{0.682} \\ 
  ARGOX & 0.243 & 0.254 & 0.273 & 0.328 & 0.377 & \textbf{0.172} & 0.331 & \textbf{0.416} & \textbf{0.286} & 0.337 & 0.113 & 0.345 & 0.776 \\ 
  VAR1 & 0.330 & 0.377 & 0.464 & 0.437 & 0.510 & 0.232 & 0.396 & 0.624 & 0.416 & 0.667 & \textbf{0.097} & 0.542 & 1.722 \\ 
  GFT & -- & -- & -- & 0.519 & 0.593 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.332 & 0.333 & 0.335 & 0.466 & 0.547 & 0.240 & 0.381 & 0.613 & 0.411 & 0.674 & 0.098 & 0.497 & 0.837 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & \textbf{0.980} & \textbf{0.976} & \textbf{0.971} & 0.957 & 0.953 & 0.918 & \textbf{0.942} & 0.980 & \textbf{0.978} & \textbf{0.991} & 0.888 & \textbf{0.945} & \textbf{0.927} \\ 
  ARGOX & 0.979 & 0.973 & 0.965 & 0.945 & 0.939 & \textbf{0.936} & 0.936 & \textbf{0.981} & 0.977 & 0.985 & 0.908 & 0.915 & 0.912 \\ 
  VAR1 & 0.951 & 0.928 & 0.895 & 0.885 & 0.872 & 0.887 & 0.871 & 0.939 & 0.954 & 0.930 & \textbf{0.921} & 0.816 & 0.776 \\ 
  GFT & -- & -- & -- & \textbf{0.976} & \textbf{0.974} & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.953 & 0.950 & 0.946 & 0.886 & 0.873 & 0.889 & 0.885 & 0.939 & 0.956 & 0.933 & 0.920 & 0.836 & 0.884 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in Virginia.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.VA}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & \textbf{0.420} & \textbf{0.487} & \textbf{0.590} & 0.347 & 0.380 & 0.323 & \textbf{0.527} & \textbf{0.658} & \textbf{0.428} & \textbf{0.602} & 0.149 & 0.298 & \textbf{1.650} \\ 
  ARGOX & 0.433 & 0.516 & 0.643 & \textbf{0.347} & \textbf{0.379} & \textbf{0.315} & 0.568 & 0.663 & 0.443 & 0.733 & 0.139 & \textbf{0.252} & 1.762 \\ 
  VAR1 & 1.241 & 1.477 & 1.837 & 1.384 & 1.517 & 0.701 & 1.061 & 1.381 & 0.992 & 2.428 & 0.267 & 1.054 & 4.934 \\ 
  GFT & -- & -- & -- & 0.784 & 0.840 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.494 & 0.583 & 0.721 & 0.393 & 0.430 & 0.338 & 0.568 & 0.753 & 0.549 & 0.976 & \textbf{0.122} & 0.294 & 1.896 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & \textbf{0.258} & \textbf{0.256} & \textbf{0.254} & \textbf{0.233} & \textbf{0.263} & 0.267 & \textbf{0.347} & 0.370 & \textbf{0.277} & \textbf{0.454} & 0.112 & 0.237 & \textbf{1.025} \\ 
  ARGOX & 0.258 & 0.260 & 0.263 & 0.236 & 0.267 & \textbf{0.262} & 0.365 & \textbf{0.352} & 0.286 & 0.510 & 0.103 & \textbf{0.204} & 1.097 \\ 
  VAR1 & 0.907 & 0.901 & 0.890 & 1.043 & 1.207 & 0.637 & 0.827 & 1.039 & 0.896 & 1.799 & 0.203 & 0.915 & 3.355 \\ 
  GFT & -- & -- & -- & 0.695 & 0.759 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.295 & 0.302 & 0.315 & 0.284 & 0.325 & 0.283 & 0.352 & 0.422 & 0.358 & 0.697 & \textbf{0.099} & 0.211 & 1.384 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & \textbf{0.950} & \textbf{0.955} & \textbf{0.956} & 0.939 & 0.933 & 0.824 & \textbf{0.845} & \textbf{0.877} & \textbf{0.925} & \textbf{0.965} & 0.642 & 0.874 & \textbf{0.913} \\ 
  ARGOX & 0.947 & 0.949 & 0.948 & 0.940 & 0.934 & \textbf{0.831} & 0.817 & 0.876 & 0.920 & 0.951 & \textbf{0.661} & \textbf{0.910} & 0.897 \\ 
  VAR1 & 0.521 & 0.454 & 0.518 & 0.617 & 0.549 & 0.604 & 0.012 & 0.373 & 0.731 & 0.362 & 0.557 & 0.508 & 0.225 \\ 
  GFT & -- & -- & -- & \textbf{0.961} & \textbf{0.959} & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.932 & 0.936 & 0.936 & 0.924 & 0.915 & 0.809 & 0.834 & 0.847 & 0.876 & 0.903 & 0.621 & 0.881 & 0.884 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in Washington.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.WA}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & \textbf{0.499} & \textbf{0.504} & \textbf{0.512} & \textbf{0.621} & \textbf{0.678} & 0.367 & 0.399 & \textbf{0.818} & 0.627 & \textbf{0.678} & 0.393 & 0.461 & \textbf{0.744} \\ 
  ARGOX & 0.519 & 0.523 & 0.530 & 0.633 & 0.690 & \textbf{0.357} & \textbf{0.389} & 0.870 & \textbf{0.614} & 0.815 & \textbf{0.384} & 0.447 & 0.760 \\ 
  VAR1 & 1.344 & 1.442 & 1.607 & 1.742 & 1.916 & 0.963 & 1.270 & 2.004 & 1.517 & 1.859 & 0.387 & 0.815 & 4.273 \\ 
  GFT & -- & -- & -- & 1.002 & 1.004 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.645 & 0.611 & 0.543 & 0.765 & 0.838 & 0.391 & 0.426 & 1.117 & 0.692 & 0.968 & 0.435 & \textbf{0.431} & 0.836 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & \textbf{0.312} & \textbf{0.319} & \textbf{0.331} & 0.412 & 0.459 & 0.309 & 0.331 & \textbf{0.509} & \textbf{0.406} & \textbf{0.396} & 0.232 & 0.360 & \textbf{0.609} \\ 
  ARGOX & 0.320 & 0.325 & 0.333 & \textbf{0.405} & \textbf{0.450} & 0.295 & 0.316 & 0.548 & 0.419 & 0.487 & 0.223 & 0.332 & 0.625 \\ 
  VAR1 & 0.843 & 0.832 & 0.811 & 1.151 & 1.360 & 0.868 & 0.902 & 1.318 & 1.118 & 1.453 & \textbf{0.210} & 0.647 & 2.912 \\ 
  GFT & -- & -- & -- & 0.915 & 0.900 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.356 & 0.352 & 0.346 & 0.491 & 0.563 & \textbf{0.281} & \textbf{0.298} & 0.665 & 0.437 & 0.659 & 0.261 & \textbf{0.285} & 0.703 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & \textbf{ 0.958} & \textbf{ 0.946} & \textbf{ 0.892} &  0.958 &  0.953 &  0.798 &  0.931 & \textbf{ 0.931} &  0.923 & \textbf{ 0.955} &  0.368 &  0.333 & \textbf{ 0.779} \\ 
  ARGOX &  0.954 &  0.941 &  0.887 &  0.956 &  0.951 & \textbf{ 0.811} & \textbf{ 0.935} &  0.922 & \textbf{ 0.927} &  0.934 & \textbf{ 0.403} &  0.297 &  0.771 \\ 
  VAR1 &  0.737 &  0.595 &  0.723 &  0.900 &  0.886 &  0.728 &  0.455 &  0.748 &  0.695 &  0.630 &  0.245 & -0.214 &  0.627 \\ 
  GFT & -- & -- & -- & \textbf{ 0.966} & \textbf{ 0.961} & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive &  0.930 &  0.922 &  0.884 &  0.930 &  0.919 &  0.798 &  0.921 &  0.872 &  0.907 &  0.910 &  0.317 & \textbf{ 0.396} &  0.712 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in West Virginia.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.WV}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & \textbf{0.371} & 0.357 & 0.329 & \textbf{0.529} & \textbf{0.562} & 0.333 & 0.396 & 0.385 & 0.270 & 0.410 & 0.126 & 0.209 & \textbf{0.394} \\ 
  ARGOX & 0.372 & \textbf{0.356} & \textbf{0.324} & 0.555 & 0.596 & \textbf{0.330} & \textbf{0.380} & \textbf{0.354} & \textbf{0.267} & \textbf{0.405} & 0.131 & \textbf{0.203} & 0.404 \\ 
  VAR1 & 0.474 & 0.445 & 0.386 & 0.759 & 0.827 & 0.351 & 0.447 & 0.552 & 0.297 & 0.616 & 0.089 & 0.232 & 0.505 \\ 
  GFT & -- & -- & -- & 0.784 & 0.842 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.446 & 0.428 & 0.392 & 0.717 & 0.781 & 0.347 & 0.424 & 0.459 & 0.294 & 0.575 & \textbf{0.085} & 0.236 & 0.486 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & 0.273 & 0.243 & 0.186 & \textbf{0.407} & \textbf{0.430} & 0.278 & 0.322 & 0.295 & 0.212 & 0.346 & 0.097 & 0.169 & \textbf{0.312} \\ 
  ARGOX & \textbf{0.271} & \textbf{0.239} & \textbf{0.181} & 0.415 & 0.445 & \textbf{0.268} & \textbf{0.319} & \textbf{0.269} & \textbf{0.211} & \textbf{0.334} & 0.103 & \textbf{0.160} & 0.314 \\ 
  VAR1 & 0.322 & 0.278 & 0.196 & 0.467 & 0.519 & 0.299 & 0.360 & 0.415 & 0.237 & 0.461 & 0.073 & 0.171 & 0.409 \\ 
  GFT & -- & -- & -- & 0.635 & 0.686 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.305 & 0.266 & 0.192 & 0.461 & 0.517 & 0.298 & 0.344 & 0.353 & 0.224 & 0.414 & \textbf{0.067} & 0.177 & 0.383 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & \textbf{0.953} & 0.954 & 0.954 & \textbf{0.935} & 0.909 & 0.737 & 0.887 & 0.947 & 0.894 & 0.965 & 0.919 & 0.896 & \textbf{0.939} \\ 
  ARGOX & 0.953 & \textbf{0.954} & \textbf{0.955} & 0.929 & 0.896 & \textbf{0.745} & \textbf{0.895} & \textbf{0.956} & \textbf{0.897} & \textbf{0.969} & 0.913 & \textbf{0.897} & 0.934 \\ 
  VAR1 & 0.931 & 0.931 & 0.937 & 0.881 & 0.816 & 0.738 & 0.866 & 0.915 & 0.880 & 0.917 & 0.931 & 0.798 & 0.903 \\ 
  GFT & -- & -- & -- & 0.896 & \textbf{0.914} & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.933 & 0.936 & 0.938 & 0.883 & 0.822 & 0.743 & 0.869 & 0.921 & 0.885 & 0.923 & \textbf{0.932} & 0.799 & 0.905 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in Wisconsin.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.WI}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & \textbf{0.487} & 0.613 & 0.795 & 0.357 & 0.392 & \textbf{0.348} & \textbf{0.533} & 0.728 & \textbf{0.735} & \textbf{0.773} & 0.254 & 0.795 & 1.812 \\ 
  ARGOX & 0.493 & \textbf{0.607} & \textbf{0.776} & \textbf{0.342} & \textbf{0.374} & 0.348 & 0.558 & \textbf{0.695} & 0.745 & 0.793 & \textbf{0.240} & \textbf{0.763} & \textbf{1.792} \\ 
  VAR1 & 0.909 & 0.994 & 1.134 & 1.372 & 1.500 & 0.779 & 0.860 & 1.139 & 0.815 & 1.230 & 0.376 & 1.416 & 2.262 \\ 
  GFT & -- & -- & -- & 0.588 & 0.596 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.551 & 0.685 & 0.881 & 0.357 & 0.391 & 0.373 & 0.582 & 0.810 & 0.825 & 0.929 & 0.256 & 0.802 & 2.118 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & \textbf{0.324} & 0.374 & 0.468 & 0.280 & 0.327 & \textbf{0.233} & \textbf{0.390} & 0.509 & 0.559 & \textbf{0.575} & 0.184 & 0.582 & 1.307 \\ 
  ARGOX & 0.326 & \textbf{0.373} & \textbf{0.460} & 0.275 & 0.318 & 0.237 & 0.416 & \textbf{0.490} & \textbf{0.558} & 0.602 & \textbf{0.175} & \textbf{0.565} & \textbf{1.307} \\ 
  VAR1 & 0.644 & 0.666 & 0.707 & 0.917 & 1.031 & 0.652 & 0.668 & 0.912 & 0.623 & 0.883 & 0.235 & 1.042 & 1.739 \\ 
  GFT & -- & -- & -- & 0.503 & 0.496 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.353 & 0.411 & 0.520 & \textbf{0.266} & \textbf{0.310} & 0.265 & 0.448 & 0.601 & 0.593 & 0.696 & 0.199 & 0.566 & 1.653 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & \textbf{0.956} & 0.926 & 0.866 & 0.939 & 0.918 & 0.891 & \textbf{0.862} & 0.954 & \textbf{0.911} & \textbf{0.913} & 0.281 & 0.696 & 0.724 \\ 
  ARGOX & 0.955 & \textbf{0.928} & \textbf{0.873} & \textbf{0.945} & \textbf{0.927} & \textbf{0.891} & 0.850 & \textbf{0.959} & 0.908 & 0.908 & \textbf{0.297} & 0.722 & 0.727 \\ 
  VAR1 & 0.847 & 0.796 & 0.744 & 0.900 & 0.886 & 0.710 & 0.632 & 0.912 & 0.888 & 0.810 & 0.241 & 0.517 & \textbf{0.882} \\ 
  GFT & -- & -- & -- & 0.877 & 0.856 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.943 & 0.911 & 0.847 & 0.940 & 0.921 & 0.881 & 0.842 & 0.938 & 0.890 & 0.871 & 0.159 & \textbf{0.731} & 0.656 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in Wyoming.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.WY}} 
\end{table*}
% latex table generated in R 4.0.1 by xtable 1.8-4 package
% Mon Jun 12 16:36:21 2023
\begin{table*}
\centering
\begingroup\scriptsize
\begin{tabular}{c|lllllllllllll}
  \hline
  & Whole period & '14-'23 & post-COVID & GFT period & '14-'15 & '15-'16 & '16-'17 & '17-'18 & '18-'19 & '19-'20 & '20-'21 & '21-'22 & '22-'23 \\ 
  \hline \hline \multicolumn{1}{l}{RMSE}\\ARGO-C & \textbf{0.296} & \textbf{0.520} & \textbf{0.780} & 0.205 & 0.217 & \textbf{0.196} & \textbf{0.357} & \textbf{0.516} & \textbf{0.196} & 1.406 & 0.192 & \textbf{0.571} & \textbf{1.128} \\ 
  ARGOX & 0.308 & 0.527 & 0.786 & \textbf{0.202} & \textbf{0.215} & 0.204 & 0.392 & 0.528 & 0.214 & \textbf{1.397} & 0.165 & 0.596 & 1.186 \\ 
  VAR1 & 1.284 & 1.751 & 2.386 & 0.941 & 0.910 & 1.384 & 1.391 & 1.102 & 1.524 & 3.637 & 0.386 & 1.543 & 4.954 \\ 
  GFT & -- & -- & -- & 0.531 & 0.554 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.406 & 0.609 & 0.868 & 0.231 & 0.243 & 0.262 & 0.393 & 0.773 & 0.324 & 1.585 & \textbf{0.085} & 0.641 & 1.338 \\ 
   \hline \hline \multicolumn{1}{l}{MAE}\\ARGO-C & \textbf{0.197} & \textbf{0.255} & 0.361 & 0.163 & 0.173 & \textbf{0.163} & \textbf{0.268} & 0.359 & \textbf{0.165} & \textbf{0.751} & 0.150 & \textbf{0.338} & \textbf{0.905} \\ 
  ARGOX & 0.201 & 0.257 & \textbf{0.360} & \textbf{0.160} & \textbf{0.170} & 0.173 & 0.283 & \textbf{0.355} & 0.177 & 0.756 & 0.133 & 0.345 & 0.978 \\ 
  VAR1 & 1.092 & 1.202 & 1.406 & 0.841 & 0.793 & 1.250 & 1.161 & 0.905 & 1.391 & 2.641 & 0.339 & 1.197 & 4.388 \\ 
  GFT & -- & -- & -- & 0.465 & 0.487 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive & 0.240 & 0.303 & 0.421 & 0.180 & 0.188 & 0.207 & 0.273 & 0.466 & 0.246 & 1.105 & \textbf{0.069} & 0.365 & 1.100 \\ 
   \hline \hline \multicolumn{1}{l}{Correlation}\\ARGO-C & \textbf{ 0.978} & \textbf{ 0.968} & \textbf{ 0.964} &  0.958 &  0.950 & \textbf{ 0.959} & \textbf{ 0.922} & \textbf{ 0.970} & \textbf{ 0.975} &  0.912 &  0.363 & \textbf{ 0.907} & \textbf{ 0.947} \\ 
  ARGOX &  0.976 &  0.967 &  0.963 & \textbf{ 0.960} &  0.952 &  0.956 &  0.904 &  0.969 &  0.970 & \textbf{ 0.916} &  0.375 &  0.893 &  0.939 \\ 
  VAR1 &  0.804 &  0.715 &  0.734 &  0.824 &  0.771 &  0.584 &  0.571 &  0.854 &  0.498 &  0.655 & -0.005 & -0.215 &  0.636 \\ 
  GFT & -- & -- & -- &  0.953 & \textbf{ 0.955} & -- & -- & -- & -- & -- & -- & -- & -- \\ 
  naive &  0.959 &  0.955 &  0.953 &  0.939 &  0.929 &  0.929 &  0.902 &  0.927 &  0.929 &  0.879 & \textbf{ 0.696} &  0.815 &  0.909 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Comparison of different methods for state-level \%ILI estimation in New York NY.  The MSE, MAE, and correlation are reported. The method with the best performance is highlighted in boldface for each metric in each period. \label{tab:state US.NYC}} 
\end{table*}

